BagFlip: A Certified Defense against Data Poisoning

Machine learning models are vulnerable to data-poisoning attacks, in which an attacker maliciously modifies the training set to change the prediction of a learned model. In a trigger-less attack, the attacker can modify the training set but not the test inputs, while in a backdoor attack the attacker can also modify test inputs. Existing model-agnostic defense approaches either cannot handle backdoor attacks or do not provide effective certificates (i.e., a proof of a defense). We present BagFlip, a model-agnostic certified approach that can effectively defend against both trigger-less and backdoor attacks. We evaluate BagFlip on image classification and malware detection datasets. BagFlip is equal to or more effective than the state-of-the-art approaches for trigger-less attacks and more effective than the state-of-the-art approaches for backdoor attacks.

==> BagFlip_ A Certified Defense against Data Poisoning/figs/bd_ember.tex <==
\centering
\tiny
    
\begin{tikzpicture}
\pgfplotsset{filter discard warning=false}
\pgfplotsset{every axis legend/.append style={
at={(1.5,1)},
anchor=north east}} 

\pgfplotscreateplotcyclelist{whatever}{%
    black,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    black,thick,dotted,every mark/.append style={fill=red!80!black},mark=none\\%
    % gray,thick,dotted, every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,dashed,every mark/.append style={fill=red!80!black},mark=none\\%
    % black,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,every mark/.append style={fill=red!80!black},mark=none\\%
    % % brown!60!black,every mark/.append style={fill=brown!80!black},mark=triangle*\\%
    % black,mark=star\\%
    % blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
    % brown!60!black,densely dashed,every mark/.append style={solid,fill=brown!80!black},mark=square*\\%
    % black,densely dashed,every mark/.append style={solid,fill=gray},mark=triangle*\\%
    % blue,densely dashed,mark=star,every mark/.append style=solid\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
    }
    \begin{groupplot}[
            group style={
                group size=1 by 1,
                horizontal sep=.05in,
                vertical sep=.05in,
                ylabels at=edge left,
                yticklabels at=edge left,
                xlabels at=edge bottom,
                xticklabels at=edge bottom,
            },
            % width=1in,
            height=1in,
            xlabel near ticks,
            ylabel near ticks,
            scale only axis,
            width=0.3*\textwidth,
            xmin=0,
            ymin=1,
            ymax=100,
            %xmax=1.1
        ]

        \nextgroupplot[
            % title=Robustness by demographic group,
            ylabel=Certifiable Accuracy,
            xmax=0.004,
            % xtick={0,1},
            % minor xtick={0.5,1.5},
            cycle list name=whatever,
            xlabel=Poisoning Amount $\assumeradii$ (\%)]
        \addplot table [x=x,y=0, col sep=comma]{data/backdoor/bd_ember.csv};
        % \addplot table [x=x,y=1, col sep=comma]{data/backdoor/bd_mnist.csv};
        \addplot table [x=x,y=0-normal, col sep=comma]{data/backdoor/bd_ember.csv};

% \legend{\technique-0.9, \technique-0.8};

%  \node (P1) at (pvgroup c5r1.north east) {};
%     \node (P2) at (pvgroup c5r1.south east) {};
%     \path (P1) -- node[right]{\pgfplotslegendfromname{singlelegend}} (P2);
    
    \end{groupplot}

\end{tikzpicture}
\caption{\technique-0.95 on EMBER against backdoor attack with $\featflipone$. Dashed lines show normal accuracy.}

==> BagFlip_ A Certified Defense against Data Poisoning/figs/bd_mnist_contagio.tex <==

    
\begin{tikzpicture}
\pgfplotsset{filter discard warning=false}
\pgfplotsset{every axis legend/.append style={
at={(1.5,1)},
anchor=north east}} 

\pgfplotscreateplotcyclelist{whatever}{%
    black,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    black,thick,dotted,every mark/.append style={fill=red!80!black},mark=none\\%
    % gray,thick,dotted, every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,dashed,every mark/.append style={fill=red!80!black},mark=none\\%
    % black,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,every mark/.append style={fill=red!80!black},mark=none\\%
    % % brown!60!black,every mark/.append style={fill=brown!80!black},mark=triangle*\\%
    % black,mark=star\\%
    % blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
    % brown!60!black,densely dashed,every mark/.append style={solid,fill=brown!80!black},mark=square*\\%
    % black,densely dashed,every mark/.append style={solid,fill=gray},mark=triangle*\\%
    % blue,densely dashed,mark=star,every mark/.append style=solid\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
    }
    \begin{groupplot}[
            group style={
                group size=2 by 1,
                horizontal sep=.05in,
                vertical sep=.05in,
                ylabels at=edge left,
                yticklabels at=edge left,
                xlabels at=edge bottom,
                xticklabels at=edge bottom,
            },
            % width=1in,
            height=.8in,
            xlabel near ticks,
            ylabel near ticks,
            scale only axis,
            width=0.2*\textwidth,
            xmin=0,
            ymin=1,
            ymax=100,
            %xmax=1.1
        ]

        \nextgroupplot[
            % title=Robustness by demographic group,
            ylabel=Certifiable Accuracy,
            xmax=1.6,
            xtick={0,1},
            minor xtick={0.5,1.5},
            cycle list name=whatever,
            xlabel=Poisoning Amount $\assumeradii$ (\%)]
        \addplot table [x=x,y=1, col sep=comma]{data/backdoor/bd_mnist.csv};
        % \addplot table [x=x,y=1, col sep=comma]{data/backdoor/bd_mnist.csv};
        \addplot table [x=x,y=1-normal, col sep=comma]{data/backdoor/bd_mnist.csv};
        
        \nextgroupplot[
            xmax=2.2,
            xtick={0,1,2},
            minor xtick={0.5,1.5},
            % title=Robustness by demographic group,
            cycle list name=whatever]
        \addplot table [x=x,y=0, col sep=comma]{data/backdoor/bd_contagio.csv};
        % \addplot table [x=x,y=1, col sep=comma]{data/backdoor/bd_contagio.csv};
        \addplot table [x=x,y=0-normal, col sep=comma]{data/backdoor/bd_contagio.csv};



% \legend{\technique-0.9, \technique-0.8};

%  \node (P1) at (pvgroup c5r1.north east) {};
%     \node (P2) at (pvgroup c5r1.south east) {};
%     \path (P1) -- node[right]{\pgfplotslegendfromname{singlelegend}} (P2);
    
    \end{groupplot}

\end{tikzpicture}

==> BagFlip_ A Certified Defense against Data Poisoning/figs/mnist_0.8_ss.tex <==
\begin{tikzpicture}
\pgfplotsset{filter discard warning=false}
\pgfplotsset{every axis legend/.append style={
at={(1.5,1)},
anchor=north east}} 

\pgfplotscreateplotcyclelist{whatever}{%
    black,thick,dotted,every mark/.append style={fill=blue!80!black},mark=none\\%
    black,thick,every mark/.append style={fill=red!80!black},mark=none\\%
    black!60,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    black!36,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    black!20,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    black!12,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,dashed,every mark/.append style={fill=red!80!black},mark=none\\%
    % black,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,every mark/.append style={fill=red!80!black},mark=none\\%
    % % brown!60!black,every mark/.append style={fill=brown!80!black},mark=triangle*\\%
    % black,mark=star\\%
    % blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
    % brown!60!black,densely dashed,every mark/.append style={solid,fill=brown!80!black},mark=square*\\%
    % black,densely dashed,every mark/.append style={solid,fill=gray},mark=triangle*\\%
    % blue,densely dashed,mark=star,every mark/.append style=solid\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
    }
    \begin{groupplot}[
            group style={
                group size=1 by 1,
                horizontal sep=.05in,
                vertical sep=.05in,
                ylabels at=edge left,
                yticklabels at=edge left,
                xlabels at=edge bottom,
                xticklabels at=edge bottom,
            },
            % width=1in,
            height=.8in,
            xlabel near ticks,
            ylabel near ticks,
            scale only axis,
            width=0.26*\textwidth,
            xmin=0,
            ymin=1,
            ymax=100,
            %xmax=1.1
        ]

        \nextgroupplot[
            % title=Robustness by demographic group,
            ylabel=Certifiable Accuracy,
            xmax=2.7,
            xtick={0,1,2},
            minor xtick={0.5,1.5,2.5},
            cycle list name=whatever,
            xlabel=Poisoning Amount $\assumeradii$ (\%)]
        \addplot table [x=x,y=0, col sep=comma]{data/trigger_less/mnist_0.8_s.csv};
        \addplot table [x=x,y=1, col sep=comma]{data/trigger_less/mnist_0.8_s.csv};
        \addplot table [x=x,y=2, col sep=comma]{data/trigger_less/mnist_0.8_s.csv};
        \addplot table [x=x,y=3, col sep=comma]{data/trigger_less/mnist_0.8_s.csv};
         \addplot table [x=x,y=4, col sep=comma]{data/trigger_less/mnist_0.8_s.csv};
          \addplot table [x=x,y=6, col sep=comma]{data/trigger_less/mnist_0.8_s.csv};



\legend{Bagging, $\featflipone$, $\featfliptwo$,$\featflipfour$, $\featflipeight$, $\featflipinf$};

%  \node (P1) at (pvgroup c5r1.north east) {};
%     \node (P2) at (pvgroup c5r1.south east) {};
%     \path (P1) -- node[right]{\pgfplotslegendfromname{singlelegend}} (P2);
    
    \end{groupplot}

\end{tikzpicture}

==> BagFlip_ A Certified Defense against Data Poisoning/figs/trigger_less_partial.tex <==
\begin{figure}[t!]
\centering
\tiny
\pgfplotsset{filter discard warning=false}
\pgfplotsset{every axis legend/.append style={
at={(1.5,1)},
anchor=north east}} 

\pgfplotscreateplotcyclelist{whatever}{%
    black,thick,dotted,every mark/.append style={fill=blue!80!black},mark=none\\%
    black,thick,every mark/.append style={fill=red!80!black},mark=none\\%
    gray,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,dashed,every mark/.append style={fill=red!80!black},mark=none\\%
    % black,thick,every mark/.append style={fill=blue!80!black},mark=none\\%
    % gray,thick,every mark/.append style={fill=red!80!black},mark=none\\%
    % % brown!60!black,every mark/.append style={fill=brown!80!black},mark=triangle*\\%
    % black,mark=star\\%
    % blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
    % brown!60!black,densely dashed,every mark/.append style={solid,fill=brown!80!black},mark=square*\\%
    % black,densely dashed,every mark/.append style={solid,fill=gray},mark=triangle*\\%
    % blue,densely dashed,mark=star,every mark/.append style=solid\\%
    % red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
    }
    
\begin{tikzpicture}
    \begin{groupplot}[
            group style={
                group size=4 by 1,
                horizontal sep=.05in,
                vertical sep=.05in,
                ylabels at=edge left,
                yticklabels at=edge left,
                xlabels at=edge bottom,
                xticklabels at=edge bottom,
            },
            % width=1in,
            height=.8in,
            xlabel near ticks,
            ylabel near ticks,
            scale only axis,
            width=0.2*\textwidth,
            xmin=0,
            ymin=0,
            ymax=100,
            %xmax=1.1
        ]

        \nextgroupplot[
            % title=Robustness by demographic group,
            ylabel=Certifiable Accuracy,
            xmax=2.7,
            xtick={0,1,2},
            minor xtick={0.5,1.5,2.5},
            cycle list name=whatever,
            xlabel=Poisoning Amount $\assumeradii$ (\%)]
        \addplot table [x=x,y=0, col sep=comma]{data/trigger_less/mnist_1.csv};
        \addplot table [x=x,y=1, col sep=comma]{data/trigger_less/mnist_1.csv};
        \addplot table [x=x,y=2, col sep=comma]{data/trigger_less/mnist_1.csv};
        
        \nextgroupplot[
            xmax=0.7,
            xtick={0,0.2,0.4,0.6},
            minor xtick={0.1,0.3,0.5,0.7},
             cycle list name=whatever,
        ]
        \addplot table [x=x,y=0, col sep=comma]{data/trigger_less/mnist_inf.csv};
        \addplot table [x=x,y=1, col sep=comma]{data/trigger_less/mnist_inf.csv};
        \addplot table [x=x,y=2, col sep=comma]{data/trigger_less/mnist_inf.csv};


        \nextgroupplot[
        xmax=0.35,
            xtick={0,0.1,0.2,0.3},
            minor xtick={0.05,0.15,0.25},
             cycle list name=whatever,
        ]
        \addplot table [x=x,y=0, col sep=comma]{data/trigger_less/ember_1.csv};
        \addplot table [x=x,y=1, col sep=comma]{data/trigger_less/ember_1.csv};
        \addplot table [x=x,y=2, col sep=comma]{data/trigger_less/ember_1.csv};
        
        \nextgroupplot[
        xmax=0.24,
            xtick={0,0.1,0.2},
            minor xtick={0.05,0.15},
             cycle list name=whatever,
        ]
        \addplot table [x=x,y=0, col sep=comma]{data/trigger_less/ember_inf.csv};
        \addplot table [x=x,y=1, col sep=comma]{data/trigger_less/ember_inf.csv};
        \addplot table [x=x,y=2, col sep=comma]{data/trigger_less/ember_inf.csv};



\legend{Bagging, \technique-$a$, \technique-$b$};

%  \node (P1) at (pvgroup c5r1.north east) {};
%     \node (P2) at (pvgroup c5r1.south east) {};
%     \path (P1) -- node[right]{\pgfplotslegendfromname{singlelegend}} (P2);
    
    \end{groupplot}
    \node[draw] at (1.45,1.7) {\scriptsize (a) MNIST $\featflipone$};
    \node[draw] at (4,0.5) {\scriptsize (b) MNIST $\featflipinf$};
    \node[draw] at (7.5,1.7) {\scriptsize (c) EMBER $\featflipone$};
    \node[draw] at (9.8,0.5) {\scriptsize (d) EMBER $\featflipinf$};

\end{tikzpicture}
\vspace{-1em}
\caption{Comparison to Bagging on MNIST and EMBER, showing the certified accuracy at different poisoning amounts $\assumeradii$. 
For MNIST: $a=0.9$ and $b=0.8$. For EMBER: $a=0.95$ and $b=0.9$.
% Normal accuracy is equal to the certified accuracy at $\assumeradii=0$ in trigger-less setting because $\poisonins_i \ge 0$. 
}
\vspace{-2em}
\label{fig:compare_bagging}
\end{figure}

==> BagFlip_ A Certified Defense against Data Poisoning/macros.tex <==
%%%%%%%%%%%%%%%%%% Notes %%%%%%%%%%%%%%%%%%
\newcommand{\mytodoblue}[1]{\textcolor{blue}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodoviolet}[1]{\textcolor{violet}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodopink}[1]{\textcolor{Maroon}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodogreen}[1]{\textcolor{Green}{\ding{46}~{\sf}~#1}}

\newcommand{\yh}[1]{\mytodopink{[yuhao: #1]}}
\newcommand{\loris}[1]{\mytodoviolet{[loris: #1]}}
\newcommand{\aws}[1]{\mytodoblue{aws---#1}}
\newcommand{\anna}[1]{\mytodogreen{anna---#1}}


\newcommand{\newadded}[1]{
\textcolor{red}{==========new BEGIN==========}

#1

\textcolor{red}{==========new END==========}
}

% \newcommand{\yh}[1]{}
% \newcommand{\loris}[1]{}
% \newcommand{\aws}[1]{}

\newcommand{\todo}[1]{{\color{red} \bf \{TODO: {#1}\}}}
\newcommand{\etal}{et al.}
\newcommand{\code}[1]{{\tt {#1}}}
\newcommand{\smalltitle}[1]{{\smallskip \noindent \bf  {#1}.\ }}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\def\modify#1#2#3{{\small\underline{\sf{#1}}:} {\color{red}{\small #2}}
{{\color{red}\mbox{$\Rightarrow$}}} {\color{blue}{#3}}}

\newcommand{\yhmodify}[2]{\modify{Yuhao}{#1}{#2}}

\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
  \do\Y\do\Z}

%%%%%%%%%%%%%%%%%% Code %%%%%%%%%%%%%%%%%%
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1,1,1}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,           
    tabsize=2,
    xleftmargin=1.5em
}

\lstset{style=mystyle}


%%%%%%%%%%%%%%%%%% Math & Symbols %%%%%%%%%%%%%%%%%%
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{proposition}{Proposition}[section]


\newcommand{\technique}{BagFlip\xspace}
\newcommand{\perturb}{\pi}
\newcommand{\alphabet}{\Sigma}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfz}{\mathbf{z}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\poisoned}[1]{\widetilde{#1}}
\newcommand{\poisonfeat}{s}
\newcommand{\poisonins}{r}
\newcommand{\Outcome}{O}
\newcommand{\outcome}{o}
\newcommand{\subspace}{\mathcal{L}}
\newcommand{\secondy}{y'}
\newcommand{\firsty}{y^*}
\newcommand{\secondp}{p'}
\newcommand{\firstp}{p^*}
\newcommand{\dis}[2]{\|#1-#2\|_0}
\newcommand{\featflip}{\textsc{f}_{\poisonfeat}}
\newcommand{\featflipone}{\textsc{f}_{1}}
\newcommand{\featflipinf}{\textsc{f}_{\infty}}
\newcommand{\labelflip}{\textsc{l}}
\newcommand{\trigger}{\perturb_{\mathrm{trig}, \poisonfeat}}
\newcommand{\featfliplabelflip}{\textsc{fl}_{\poisonfeat}}
\newcommand{\featfliplabelflipone}{\textsc{fl}_{1}}
\newcommand{\featfliptwo}{\textsc{f}_{2}}
\newcommand{\featflipfour}{\textsc{f}_{4}}
\newcommand{\featflipeight}{\textsc{f}_{8}}
\newcommand{\featflipsixteen}{\textsc{f}_{16}}
% \newcommand{\selectflip}{\mu_{\mathrm{bf}}}
\newcommand{\selectflip}{\mu}
\newcommand{\selectwords}{\mu_{\mathrm{sw}}}
\newcommand{\bfxtest}{\bfx}
\newcommand{\ytest}{y}
\newcommand{\alg}{A}
\newcommand{\ualg}{A^?}
\newcommand{\salg}{\bar{\alg}}
\newcommand{\sualg}{\bar{\ualg}}
% \newcommand{\model}[1]{A_{#1}}
\newcommand{\modelpredo}[1]{\alg(#1)}
\newcommand{\umodelpredo}[1]{\ualg(#1)}
\newcommand{\modelpred}[2]{\alg(#1,#2)}
% \newcommand{\smodel}[1]{\salg_{#1}}
\newcommand{\smodelpred}[2]{\salg(#1,#2)}
\newcommand{\poisonset}[1]{S^{#1}_r(D)}
\newcommand{\lb}{\mathrm{lb}}
\newcommand{\ub}{\mathrm{ub}}
\newcommand{\sample}[1]{\dot{#1}}
\newcommand{\poisondist}{\poisoned{\mu}}
\newcommand{\cleandist}{\mu}
\newcommand{\lbsubset}{\mathcal{S}^*}
\newcommand{\ubsubset}{\mathcal{S}'}
\newcommand{\assumeradii}{R}
\newcommand{\symbolremain}{\rho}
\newcommand{\symbolflip}{\gamma}
\newcommand{\indexset}{B}
\newcommand{\smallk}{\kappa}
\newcommand{\diffu}{\Delta}
\newcommand{\diffv}{\poisoned{\Delta}}
\newcommand{\cleandistmass}[1]{p_{\cleandist}(#1)}
\newcommand{\poisondistmass}[1]{p_{\poisondist}(#1)}

\newcommand{\PP}{\mathrm{Pr}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\EE}{\mathds{E}}

==> BagFlip_ A Certified Defense against Data Poisoning/pkgs.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage[group-separator={,}]{siunitx}
\usepackage{booktabs} % For formal tables
\usepackage{color}
\usepackage{listings}
\usepackage{enumitem}
\usepackage{threeparttable}
\usepackage{multirow}% http://ctan.org/pkg/multirow
\usepackage{hhline}% http://ctan.org/pkg/hhline
\usepackage{subfigure}
\usepackage{array}
\usepackage{pifont}
\usepackage{booktabs}
\usepackage{dsfont}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{stmaryrd}
\usepackage{amsmath}
\let\Bbbk\relax
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{url}
\usepackage{bbm}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage{booktabs, siunitx}
\usepackage[svgnames,table]{xcolor}
\usepackage[tableposition=above]{caption}
\usepackage{xcolor}
\usepackage{tkz-euclide}
\usepackage[framemethod=tikz]{mdframed}
\usepackage{empheq}
\usepackage[most]{tcolorbox}
\usepackage{adjustbox}
\usepackage{wrapfig}
\usepackage{hyperref}
\usepackage[capitalize]{cleveref}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}


\usepackage{balance}
\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
  \do\Y\do\Z}


==> BagFlip_ A Certified Defense against Data Poisoning/sections/abstract.tex <==
\begin{abstract}
Machine learning models are vulnerable to data-poisoning attacks, in which an attacker maliciously modifies the training set to change the prediction of a learned model. 
In a \emph{trigger-less} attack, the attacker can modify the training set but not the test inputs, while in a \emph{backdoor} attack the attacker can also modify test inputs. 
Existing model-agnostic defense approaches either cannot handle backdoor attacks or do not provide effective certificates (i.e., a proof of a defense).
We present \technique, a model-agnostic certified approach that can effectively defend against both trigger-less and backdoor attacks. 
We evaluate \technique on image classification and malware detection datasets. 
\technique is equal to or more effective than the state-of-the-art approaches for trigger-less attacks and more effective than the state-of-the-art approaches for backdoor attacks. 
\end{abstract}


==> BagFlip_ A Certified Defense against Data Poisoning/sections/approach.tex <==
\section{\technique: Dual-Measure Randomized Smoothing}
\label{sec:smoothing}

% \aws{give a catchy/descriptive name to the approach}
Our approach, which we call \technique, is a model-agnostic certification technique.
Given a learning algorithm $\alg$, we want to automatically construct a new learning algorithm $\salg$ with certified poisoning-robustness guarantees (\cref{eq:trigger_less_goal,eq:goal}).
To do so, we adopt and extend the framework of \emph{randomized smoothing}.
Initially used for test-time robustness, randomized smoothing robustifies a function $f$ by carefully constructing a \emph{noisy} version $\bar{f}$ and theoretically analyzing the guarantees of $\bar{f}$.

Our approach, \technique, constructs a noisy algorithm $\salg$ by randomly
perturbing the training set and the test input and invoking $\alg$ on the result.
Formally, if we have a set of output labels $\mathcal{C}$, we define the \emph{smoothed} learning algorithm $\salg$ as follows:
\begin{align}
\smodelpred{D}{\bfxtest} \triangleq \underset{y\in \mathcal{C}}{\mathrm{argmax}} \underset{\sample{D}, \sample{\bfxtest} \sim \mu(D, \bfxtest)}{\PP}(\modelpred{\sample{D}}{\sample{\bfxtest}}=y), \label{eq:smoothing1}    
\end{align}
where $\mu$ is a carefully designed probability distribution---the \emph{smoothing distribution}---%
over the training set and the test input ($\sample{D}, \sample{\bfxtest}$ are a sampled dataset and a test input from the smoothing distribution).
 
%  \aws{rearranged to somewhat what it was before ... not sure what's better}

We present two key contributions that enable \technique to efficiently certify robustness up to large poisoning radii.
First, we define a smoothing distribution $\selectflip$ that combines \emph{bagging}~\cite{bagging} of the training set $D$, and noising~\cite{featureflip} of the training set and the test input $\bfx$ (done by randomly \emph{flipping} features and labels). This combination, described below, allows us to defend against trigger-less and backdoor attacks.
%
However, this combination also makes it challenging to compute the certified radius
due to the combinatorial explosion of the sample space.
Our second contribution is a partition strategy for the Neyman--Pearson lemma that results in an efficient certification algorithm (\cref{sec:precise_approach}), as well as a relaxation of the Neyman--Pearson lemma that further speeds up certification (\cref{sec:imprecise}).


% \aws{modified, please check}
\textbf{Smoothing distribution.}
We describe the smoothing distribution $\selectflip$ that defends against feature and label flipping.
Given a dataset $D = \{(\bfx_i, y_i)\}$ and a test input $\bfxtest$, sampling from 
$\selectflip(D,\bfx)$ generates a random dataset and test input in the following way:
(1) Uniformly select $k$ examples from $D$ with replacement and record their indices as $w_1, \ldots, w_k$. (2) 
Modify each selected example $(\bfx_{w_i},y_{w_i})$ and the test input $\bfxtest$ to $(\bfx_{w_i}',y_{w_i}')$ and $\bfxtest'$, respectively, as follows: For each feature, with probability $1-\symbolremain$,
uniformly change its value to one of the other categories in $\{0,\ldots,K\}$.
Randomly modify labels $y_{w_i}$ in the same way.
%
In other words, each feature will be \emph{flipped} to another value from the domain 
with probability $\symbolflip \triangleq \frac{1 - \symbolremain}{K}$,
where $\symbolremain \in [0, 1]$ is the parameter controlling the noise level. 

For $\featflip$ (resp. $\labelflip$), we simply do not modify the labels (resp. features) of
the $k$ selected examples. 
\begin{example}
\label{exp: distribution}
Suppose we defend against $\featflipone$ in a trigger-less setting, then the distribution $\selectflip$ will not modify labels or the test input. Let $\symbolremain = \frac{4}{5}$, $k=1$.
Following \Cref{exp: perturbation}, let the binary-classification image dataset $D=\{(\bfx_1, y_1), (\bfx_2, y_2)\}$, 
where each image contains only one pixel. 
Then, one possible element of $\selectflip(D, \bfxtest)$ can be the pair $(\{(\bfx_2', y_2)\}, \bfxtest)$, where $\bfx_2' = \bfx_2$.
The probability of this element is $\frac{1}{2} \times \symbolremain = 0.4$ because we uniformly select one out of two examples and do not flip any feature, that is, the single feature retains its original value. 
\end{example}





==> BagFlip_ A Certified Defense against Data Poisoning/sections/conclusion.tex <==
\section{Conclusion, Limitations, and Future Work}
\label{sec: conclusion}
We presented \technique, a certified probabilistic approach that can effectively defend against both trigger-less and backdoor attacks.
We foresee many future improvements to \technique. First, \technique treats both the data and the underlying machine learning models as closed boxes. Assuming a specific data distribution and training algorithm can further improve the computed certified radius. 
Second, \technique uniformly flips the features and the label, while it is desirable to adjust the noise levels for the label and important features for better normal accuracy according to the distribution of the data. 
Third, while probabilistic approaches need to retrain thousands of models after a fixed number of predictions, the deterministic approaches can reuse models for every prediction. Thus, it is interesting to develop a deterministic model-agnostic approach that can defend against both trigger-less and backdoor attacks.


==> BagFlip_ A Certified Defense against Data Poisoning/sections/efficient_theorem.tex <==
\section{An Efficient Relaxation for Computing a Certified Radius}
\label{sec:imprecise}
Theorem~\ref{thm:np_bound} requires computing the likelihood ratio of a large number of subspaces $\subspace_1,\ldots,\subspace_m$.
We propose a generalization of the Neyman--Pearson lemma that \textbf{underapproximates} the subspaces by a small subset and computes a lower bound $\lb_\delta$ for $\lb$.
We then show how to choose a subset of subspaces that yields a tight underapproximation. 

% \begin{figure}[t]
%     \centering
%      \includegraphics[width=\columnwidth]{figs/np_illustration.png}
%     \caption{Illustrations of Theorem~\ref{thm:np_bound} and Theorem~\ref{thm:np_non_tight}.\todo{refine}}
%     \label{fig:np_lemmas}
% \end{figure}

\textbf{A relaxation of the Neyman--Pearson lemma.}
The key idea is to use Theorem~\ref{thm:np_bound} to examine only a \textit{subset} of the subspaces $\{\subspace_i\}_i$.
Suppose that we partition the subspaces $\{\subspace_i\}_i$ into two sets $\{\subspace_i\}_{i\in \indexset}$
and $\{\subspace_i\}_{i\not\in \indexset}$, using 
a set of indices $\indexset$.
We define a new lower bound $\lb_\delta$ by applying Theorem~\ref{thm:np_bound} to the first group $\{\subspace_i\}_{i\in \indexset}$ and underapproximating $\firstp$ in Theorem~\ref{thm:np_bound} as $\firstp - \sum_{i\notin \indexset} \cleandistmass{\subspace_i}$.
Intuitively, the underapproximation ensures that any subspace in $\{\subspace_i\}_{i\not\in \indexset}$ will not contribute to the lower bound, even though these subspaces may have contributed to the precise $\lb$ computed by Theorem~\ref{thm:np_bound}.

The next theorem shows that $\lb_\delta$ will be smaller than $\lb$ by an error term $\delta$ that is a function of the partition $\indexset$.
The gain is in the number of subspaces we have to consider, which is now $|B|$.

\begin{theorem}[Relaxation of the Lemma]
\label{thm:np_non_tight}
% Suppose the original likelihood ratios are $\eta_1 \ge \ldots \eta_m$ corresponding to subspaces $\subspace_1, \ldots, \subspace_m$ and we partition the subspaces into two groups $\subspace_\indexset$ and $\subspace_{\neg \indexset}$. 
Define $\lb$ for the subspaces $\subspace_1, \ldots, \subspace_m$ as in \cref{thm:np_bound}.
Define $\lb_\delta$ for $\{\subspace_i\}_{i\in \indexset}$ as in \cref{thm:np_bound}  
by underapproximating $\firstp$ as 
$\firstp - \sum_{i\notin \indexset} \cleandistmass{\subspace_i}$, then we have 
\textbf{Soundness:} $\lb_\delta \le \lb$ and \textbf{$\delta$-Tightness:} Let $\delta \triangleq \sum_{i \notin \indexset} \poisondistmass{\subspace_i}$, then $\lb_\delta + \delta \ge \lb$.
% \[\lb_\delta \le \underset{\outcome \sim \poisondist}{\PP}(\modelpredo{\outcome}=\firsty) \le \lb_\delta + \delta^*,\quad \ub_\delta \ge \underset{\outcome\sim \poisondist}{\PP}(\modelpredo{\outcome}=\secondy) \ge \ub_\delta - \delta',\]
% where the non-tightness $\delta^*$ and $\delta'$ are defined as 
% \[\delta^* = \sum_{i=l+1}^m \underset{\outcome \sim \cleandist}{\PP}(\outcome \in \subspace_{i}),\quad \delta' = \sum_{i=l+1}^m  \underset{\outcome \sim \poisondist}{\PP}(\outcome \in \subspace_{i})\]
\end{theorem}

\begin{example}
\label{exp: relaxation}
Consider $\subspace_1, \subspace_2$, and $\subspace_3$ from \Cref{exp: lemma}. If we set $\indexset = \{1, 2\}$ and underapproximate $\firstp$ as $\firstp - \cleandistmass{\subspace_3} = 0.85$,
then we have $\lb_\delta = 0.1 + (0.85 - 0.4) / 1 = 0.55$, which can still certify Eq.~\ref{eq:certgoal1}.
However, $\lb_\delta$ is not close to the original $\lb = 0.8$ because the error $\delta = 0.4$ is large in this example.
Next, we will show how to choose $\indexset$ as small as possible while still keeping $\delta$ small. 
\end{example}

\textbf{Speeding up radius computation.}
The total time for computing $\lb$ consists of two parts, (1) the efficient algorithm~(Eq~\ref{eq:efficient_tct}) computes $T(c,t)$ in $O(d^3+k^2d^2)$, and (2) Theorem~\ref{thm:np_bound} takes $O(k^2d)$ for a given $\firstp$ because there are $O(k^2d)$ subspaces. 
Even though we have made the computation polynomial by the above two techniques in \cref{sec: featflip}, it can still be slow for large bag sizes $k$, which can easily be in hundreds or thousands.


We will apply Theorem~\ref{thm:np_non_tight} to replace the bag size $k$ with a small constant $\smallk$.
Observe that $\cleandistmass{\subspace_{c,t}}$ and $\poisondistmass{\subspace_{c,t}}$, as defined in \cref{sec: featflip}, are negligible for large $c$, i.e., the number of perturbed indices in the smoothed dataset.
Intuitively, if only a small portion of the training set is perturbed, it is unlikely that we select a large number of perturbed indices in the smoothed dataset.
We underapproximate the full subspaces to $\{\subspace_{c,t}\}_{(c,t) \in \indexset}$ by choosing the set of indices $\indexset=\{(c,t) \mid c\le \smallk , |t| \le (c+1)d\}$, where $\smallk$ is a constant controlling the error $\delta$, which can be computed as $\delta = \sum_{i \notin \indexset}\poisondistmass{\subspace_i} = 1 - \sum_{c=0}^\smallk \mathrm{Binom}(c;k,\frac{\poisonins}{n})$.
Theorem~\ref{thm:np_non_tight} reduces the number of subspaces to $|\indexset| = O(\smallk^2d)$.
As a result, all the $k$ appearing in previous time complexity can be replaced with $\smallk$.
\begin{example}
Suppose $k=150$ and $\frac{r}{n}=0.5\%$, choosing $\smallk = 6$ leads to $\delta = 1.23\times 10^{-5}$. 
In other words, it speeds up almost 625X for computing $T(c,t)$ and for applying Theorem~\ref{thm:np_bound}.
\end{example}



% Then we are ready to give the main theorem.
% \begin{theorem}
% \label{thm:np_bound}
% Sort the likelihood ratios descendingly, 
% \[\eta(c_1, u_1, v_1) \ge \eta(c_2, u_2, v_2) \ge \ldots \ge \eta(c_m, u_m, v_m),\]
% where $m$ is the total number of disjoint $\subspace$'s.
% Then the lower bound $lb$ can be computed as
% \begin{align}
%     lb = \underset{(D',\bfx')\sim \mu(D,\bfxtest)}{\PP}\left((D', \bfx') \in S\right) + \frac{p - \underset{(D'', \bfx'')\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left((D'', \bfx'') \in  S\right)}{\eta(c_{i_l}, u_{i_l}, v_{i_l})},\label{eq:np_bound_eqlb}
% \end{align}
% where 
% \[S = \bigcup_{j=1}^{i_l-1} \subspace(c_{j}, u_{j}, v_{j}),\quad p = \underset{(D'', \bfx'')\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}(f(D'',\bfx'')=y^*)\]
% and $i_l$ is the largest index such that 
% \[\underset{(D'', \bfx'')\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left((D'', \bfx'') \in S\right) < p\]

% Similarly, the upper bound $ub$ can be computed as
% \begin{align}
%     ub = \underset{(D',\bfx')\sim \mu(D,\bfxtest)}{\PP}\left((D', \bfx') \in R\right) + \frac{\bar{p} - \underset{(D'', \bfx'')\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left((D'', \bfx'') \in R\right)}{\eta(c_{i_u}, u_{i_u}, v_{i_u})},\label{eq:np_bound_equb}
% \end{align}
% where 
% \[R = \bigcup_{j=i_u+1}^{m} \subspace(c_{j}, u_{j}, v_{j}),\quad \bar{p} = \max_{y\neq y^*} \underset{(D'', \bfx'')\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}(f(D'',\bfx'')=y)\]
% and $i_u$ is the smallest index such that 
% \[\underset{(D'', \bfx'')\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left((D'', \bfx'') \in R\right) < \bar{p}\]
% \end{theorem}
% The above theorem is a direct application of Lemma~\ref{lemma:neyman_pearson}.

% Algorithm~\ref{alg:comp_lb} presents how to compute $lb$ using Theorem~\ref{thm:efficient} and Theorem~\ref{thm:np_bound} in polynomial time.

% \begin{algorithm}
% % \todo{further tighten the algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \caption{Compute $lb$}\label{alg:comp_lb}
% \begin{algorithmic}
% \Require $|D|, d, k, \poisonins, \poisonfeat, p, a, b (b<a)$
% \Ensure $lb$
% \State Compute $|L(u,v;\poisonfeat)|$ for all $0 \le u, v \le d$ \Comment{$O(d^3)$}
% \State Initialize $T(c,t) \gets 0$ for all $0 \le c \le k, -kd \le t \le kd$
% \State $T(0,0) \gets 1$\Comment{Compute $T(0,\cdot)$}

% \State $T(1,t) \gets \sum_{u=\max(0,t)}^{\min(d,t+d)} |L(u, u-t;s)|b^u a^{d-u}$ for all $-d \le t \le d$\Comment{Compute $T(1,\cdot)$ in $O(d^2)$}

% \For{$c = 2 \ldots k$}\Comment{Compute $T(c,\cdot)$ in $O(d^2k^2)$}
%     \State $T(c,t) \gets \sum_{t_1=\max(-d, t-(c-1)d)}^{\min(d, t+(c-1)d)} T(c-1,t - t_1)T(1,t_1)$ for all $-cd \le t \le cd$
%     % \For{$t_1 = -(c-1)d \ldots (c-1)d$}
%     %     \For{$t_2 = -d \ldots d$} 
%     %         \State $T(c,t_1+t_2) \gets T(c,t_1+t_2) + T(c-1,t_1)T(1,t_2)$
%     %     \EndFor
%     % \EndFor
% \EndFor

% \State $lb \gets 0$
% \For{$t = -kd \ldots kd$}\Comment{Apply Theorem~\ref{thm:np_bound} in $O(k^2d)$}
%     \State $\eta \gets \left(\frac{b}{a}\right)^t$
%     \For{$c = 0 \ldots k$}
%         \State $p_1 \gets F(c;k,\frac{\poisonins}{n})T(c,t)$ \Comment{$\underset{\outcome\sim \mu(\poisoned{D}, \bfxtest)}{\PP}\left(\outcome \in \subspace_{c,t}\right)$}
%         \State $p_2 \gets \frac{p_1}{\eta}$\Comment{$\underset{\outcome\sim \mu(D, \bfxtest)}{\PP}\left(\outcome \in \subspace_{c,t}\right)$}
%         \If{$p_1 < p$}
%             \State $p \gets p - p_1$
%             \State $lb \gets lb + p_2$
%         \Else 
%             \State $p \gets 0$
%             \State $lb \gets lb + \frac{p}{\eta}$
%         \EndIf
%     \EndFor
% \EndFor
% \State \Return $lb$

% % \State \Return $lb$
% \end{algorithmic}
% \end{algorithm}


% \subsection{Applying Theorem~\ref{thm:np_bound} to Distribution $\selectwords$ under Perturbation $\trigger$}
% \label{sec: trigger-words}
% \yh{this section can go to appendix}
% According to $\trigger$, the perturbed instances in dataset $\poisoned{D}$ have length of $L+\poisonfeat$, where the attacker have added trigger words of length $\poisonfeat$. 
% No matter where the trigger words are located, we can prove that there is at least $\binom{L}{l}/\binom{L+s}{l}$ probability of excluding all the trigger words when we randomly select $l$ words.

% We follow the same path as in Section~\ref{sec: featflip}, where we first partition the space $\Omega$ into disjoint subspaces $\subspace(c)$ as,
% \begin{align}
%     \subspace(c) = \{&(w_1,\bfz_1, \ldots, w_k, \bfz_k, \bfz_0)\mid \nonumber\\
%     &\sum_{i=1}^k \mathds{1}_{w_i \le \poisonins}=c ,\label{eq:Ldef1_wordattack} \\
%     &\forall 0 \le i \le k.\ \bfz_i\text{ does not contain trigger words}\},\label{eq:Ldef2_wordattack}
% \end{align}
% where Eq~\ref{eq:Ldef1_wordattack} means that there are $c$ perturbed instance being selected in the bag and Eq~\ref{eq:Ldef2_wordattack} means that selected words do not contain any of the trigger words for each training and test instance.

% Then, we directly compute the likelihood of $ \outcome \sim \selectwords(\poisoned{D}, \bfxtest)$ being in the subspace $\subspace(c)$ as 
% \[\underset{\outcome\sim \selectwords(\poisoned{D}, \bfxtest)}{\PP}\left(\outcome \in \subspace(c)\right) = F(c;k,\frac{r}{n}) \left(\dfrac{\binom{L}{l}}{\binom{L+s}{l}}\right)^{c+1}\]
% And, the likelihood of the outcomes sampling from $ \selectwords(\poisoned{D}, \bfxtest)$ is
% \[\underset{\outcome \sim \selectwords(D, \bfxtest)}{\PP}\left(\outcome \in \subspace(c)\right) = F(c;k,\frac{r}{n}),\]
% because every sentence sampled from the clean dataset is clean. 
% The likelihood ratio $\eta(c) = \binom{L}{l} / \binom{L+s}{l}$ decreases as $c$ goes larger. 
% We can sort the likelihood ratios descendingly and compute $lb$ and $ub$ by Theorem~\ref{thm:np_bound} in polynomial time.



==> BagFlip_ A Certified Defense against Data Poisoning/sections/experiments.tex <==
\section{Experiments}
\label{sec: experiment}
The implementation of \technique is publicly available\footnote{\url{https://github.com/ForeverZyh/defend_framework}}.
In this section, we evaluate \technique against trigger-less and backdoor attacks and compare \technique with existing work.
Note that we apply the relaxation in Section~\ref{sec:imprecise} to \technique in all experiments and set $\delta = 10^{-4}$.
% \begin{itemize}
%     \item \textbf{RQ1:} How does \technique perform under the trigger-less attack setting?
%     \item \textbf{RQ2:} How does \technique perform under the backdoor attack setting?
%     % \item \textbf{RQ3:} How does our framework compare to the feature-flipping approaches~\cite{featureflip, RAB}?
%     % \item \textbf{RQ4:} How does our framework perform under existing data poisoning attacks?
% \end{itemize}

\textbf{Datasets.}
We conduct experiments on MNIST, CIFAR10, EMBER~\cite{ember}, and Contagio (\url{http://contagiodump.blogspot.com}).
MNIST and CIFAR10 are datasets for image classification. EMBER and Contagio are datasets for malware detection,
where data poisoning can lead to disastrous security consequences.
To align with existing work, we select subsets of MNIST and CIFAR10 as MNIST-17, MNIST-01, and CIFAR10-02 in some experiments, e.g., MNIST-17 is a subset of MNIST with classes 1 and 7. 
We discretize all the features when applying \technique.
We use clean datasets except in the comparison with RAB~\cite{RAB}, where we follow their experimental setup and use backdoored datasets generated by BadNets~\cite{badnets}.
A detailed description of the datasets is in \Cref{sec: appendix_data}.

\textbf{Models.} We train neural networks for MNIST, CIFAR10, EMBER and random forests for Contagio. 
Unless we specifically mention the difference in some experiments, 
whenever we compare \technique to an existing work, we will use the same network structures, hyper-parameters, and data augmentation as the compared work, and we train $N=1000$ models and set the confidence level as $0.999$ for each configuration.
All the configurations we used can be found in the implementation. 

\textbf{Metrics.}
For each test input $(\bfxtest_i, y_i)$, algorithm $\salg$ will predict a label and the certified radius $\poisonins_i$.
% Assuming the attack had poisoned $R$ examples in the training set, there are three outcomes of the prediction $\smodelpred{D}{\bfxtest}$: 1) \textit{certified correct}, which means the prediction is correct and the certified radius is no less than $R$, formally $\smodelpred{D}{\bfxtest} = y \wedge \poisonins \ge R$, 2) the algorithm \textit{abstains}, formally $\poisonins < R$, and 3) \textit{certified but wrong}, which means the prediction is a wrong and the algorithm does not abstain, formally $\smodelpred{D}{\bfxtest} \neq y \wedge \poisonins \ge R$.
Assuming that the attacker had poisoned $\assumeradii\%$ of the examples in the training set, we define \textbf{certified accuracy} as the percentage of test inputs that are correctly classified and their certified radii are no less than $\assumeradii$, i.e., $\sum_{i=1}^m \mathds{1}_{\smodelpred{D}{\bfxtest_i} = y_i \wedge \frac{\poisonins_i}{n} \ge \assumeradii\%}$.
We define \textbf{normal accuracy} as the percentage of test inputs that are correctly classified, i.e., $\sum_{i=1}^m \mathds{1}_{\smodelpred{D}{\bfxtest_i} = y_i}$.

\subsection{Defending Against Trigger-less Attacks}
Two model-agnostic certified approaches, Bagging~\cite{bagging} and LabelFlip~\cite{labelflip}, can defend against trigger-less attacks.
\technique outperforms LabelFlip (comparison in~\Cref{sec: appendix_res}).
We evaluate \technique on the perturbation $\featflip$ using MNIST, CIFAR10, EMBER, and Contagio and compare \technique to Bagging. We provide comparisons with Bagging on other perturbation spaces in~\Cref{sec: appendix_res}.

We present \technique with different noise levels (different probabilities of $\symbolremain$ when flipping), denoted as \technique-$\symbolremain$.
When comparing to Bagging, we use the same $k$, the size of sampled datasets, for a fair comparison.
Furthermore, we tune the parameter $k$ in Bagging to match the normal accuracy with the \technique-$\symbolremain$ setting, and denote this setting as Bagging-$\symbolremain$.
Concretely, we set $k=100, 1000, 300, 30$ for MNIST, CIFAR10, EMBER, and Contagio respectively when comparing to Bagging. 
We tune $k=80, 280$ for Bagging-0.9 on MNIST and Bagging-0.95 on EMBER, respectively.
And we set $k=50$ for MNIST when comparing to LabelFlip.

\input{figs/trigger_less_partial}

\input{tables/trigger_less_res}

\textbf{Comparison to Bagging.} 
Bagging on a discrete dataset is a special case of \technique when $\symbolremain=1$, i.e., no noise is added to the dataset. (We present the results of bagging on the original dataset (undiscretized) in 
\Cref{sec: appendix_res}).
Table~\ref{tab:trigger_less_res} and Fig~\ref{fig:compare_bagging} show the results of \technique and Bagging on perturbations $\featflipone$ and $\featflipinf$ over MNIST and EMBER. 
The results of CIFAR10 and Contagio are similar and shown in \Cref{sec: appendix_res}.
$\featflipone$ only allows the attacker to modify one feature in each training example, and $\featflipinf$ allows the attacker to modify each training example arbitrarily without constraint.
For $\featflipone$ on MNIST, \technique-0.9 performs better than Bagging after $\assumeradii = 0.19$ and \technique-0.8 still retains non-zero certified accuracy at $\assumeradii=2.5$ while Bagging's certified accuracy drops to zero after $\assumeradii=0.66$.
We observe similar results on EMBER for $\featflipone$ in Table~\ref{tab:trigger_less_res}, except $\assumeradii=0.13$ when compared to Bagging-0.95.
We argue that it is possible to tune a best combination of $k$ and $\symbolremain$ for \technique, like we tune $k$ for Bagging-0.95, and achieve a better result while maintaining similar normal accuracy. 
However, we do not conduct hyperparameter-tuning for \technique because of its computation cost.
\textbf{\technique achieves higher certified accuracy than Bagging when the poisoning amount is large for $\featflipone$.}

For $\featflipinf$ on MNIST, Bagging performs better than \technique across all $\assumeradii$ because the noise added by \technique to the training set hurts the accuracy. 
However, we find that the noise added by \technique helps it perform better for $\featflipinf$ on EMBER.
Specifically, \technique achieves similar certified accuracy as Bagging at small radii and \technique performs better than Bagging after $\assumeradii=0.15$.
\textbf{Bagging achieves higher certified accuracy than \technique for $\featflipinf$. Except in EMBER, \technique achieves higher certified accuracy than Bagging when the amount of poisoning is large.}

% \begin{wrapfigure}{R}{0.43\textwidth}
%     \include{figs/mnist_0.8_s}
%   \label{fig:mnist_0.8_s}
  
%   \include{figs/bd_mnist_contagio}
%   \label{fig:bd_mnist_contagio}
% \end{wrapfigure}


\begin{figure}[t]
    \centering\tiny
    \subfigure{\input{figs/mnist_0.8_ss}\label{fig:mnist_0.8_s}}
    \hspace{1em}
    \subfigure{\input{figs/bd_mnist_contagio}\label{fig:bd_mnist_contagio}}
    \vspace{-1em}
    \caption{(a) \technique-0.8 on MNIST against $\featflip$ with different $\poisonfeat$. $\poisonfeat=8$ almost overlaps with $\poisonfeat=\infty$. (b) \technique-0.8 on MNIST and \technique-0.9 on Contagio against backdoor attack with $\featflipone$. Dashed lines show normal accuracy.}
    % \label{fig: treetrans}
    \vspace{-2em}
\end{figure}


We also study the effect of different $\poisonfeat$ in the perturbation function $\featflip$. 
Figure~\ref{fig:mnist_0.8_s} shows the result of \technique-0.8 on MNIST.
\technique has the highest certified accuracy for $\featflipone$. 
As $\poisonfeat$ increases, the result monotonically converges to the curve of \technique-0.8 in Figure~\ref{fig:compare_bagging}(b).
Bagging neglects the perturbation function and performs the same across all $\poisonfeat$.  
% 
Bagging performs better than \technique-0.8 when $\poisonfeat\geq 8$.
%
Other results for different datasets and different noise levels follow a similar trend (see \Cref{sec: appendix_res}).
\textbf{\technique performs best at $\featflipone$ and monotonically degenerates to $\featflipinf$ as $\poisonfeat$ increases.}

\subsection{Defending Against Backdoor Attacks}

Two model-agnostic certified approaches, FeatFlip~\cite{featureflip} and RAB~\cite{RAB}, can defend against backdoor attacks.
We compare \technique to FeatFlip on MNIST-17 perturbed using $\featfliplabelflipone$, and compare \technique to RAB on poisoned MNIST-01 and CIFAR10-02 (by BadNets~\cite{badnets}) perturbed using $\featflipone$.
We further evaluate \technique on the perturbation $\featflipone$ using MNIST and Contagio, on which existing work is unable to compute a meaningful certified radius.

% \loris{maybe remove this paragraph}
% We note that defending against backdoor attacks is strictly harder than trigger-less attack because attackers can also backdoor the test input.
% Specifically, the certified accuracy at $\assumeradii=0$ can be interpreted as the \textbf{certified evasion accuracy} against adversarial evasion attacks because Eq~\ref{eq:goal} degenerates to evasion robustness when $\poisoned{D} = D$, i.e., the training set is clean.

% However, we may not be able to certify Eq~\ref{eq:goal} when $\assumeradii=0$ in some cases
% However, normal accuracy can be greater than the certified accuracy at $\assumeradii=0$ in the backdoor setting because we define $\poisonins_i = -1$ when the 
% In the backdoor setting, the certified accuracy at $\assumeradii=0$ can be interpreted as the \textbf{certified evasion accuracy} against adversarial evasion attacks because Eq~\ref{eq:goal} degenerates to evasion robustness when $\poisoned{D} = D$.

\begin{wraptable}{R}{0.5\textwidth}
\vspace{-1.4em}
\include{tables/backdoor_res}
\label{tab:backdoor_res}
\vspace{-2em}
\end{wraptable}

\textbf{Comparison to FeatFlip.} FeatFlip scales poorly compared to \technique because its computation of the certified radius is polynomial in the size of the training set. \technique's computation is polynomial in the size of the bag instead of the size of the whole training set, and it uses a relaxation of the Neyman--Pearson lemma for further speed up.
\textbf{\technique is more scalable than FeatFlip.}

We directly cite FeatFlip's results from~\citet{featureflip} and note that FeatFlip is evaluated on a subset of MNIST-17.
As shown in Table~\ref{tab:backdoor_res}, \technique achieves similar normal accuracy, but much higher certified accuracy across all $\assumeradii$~(see full results in \Cref{sec: appendix_res}) than FeatFlip.
\textbf{\technique significantly outperforms FeatFlip against $\featfliplabelflipone$ on MNIST-17.}
% \technique-0.95 (\technique-0.9) achieves 97.5\%~(97.2\%) normal accuracy and 86.5\%~(71.6\%) certified evasion accuracy against $\featfliplabelflipone$ on MNIST-17, respectively, while FeatFlip achieves 98\% normal accuracy and 82\% certified evasion accuracy~($\assumeradii=0$).
% The certified accuracy of \technique-0.95 (\technique-0.9) retains 78.7\%~(54.1\%) at $\assumeradii=50$, respectively.
% FeatFlip achieves 36\% certified accuracy at $\assumeradii=1$ and its certified accuracy drops to zero after $\assumeradii=3$.


\textbf{Comparison to RAB.} RAB assumes a perturbation function that perturbs the input within an $l_2$-norm ball of radius $\poisonfeat$. We compare \technique to RAB on $\featflipone$, where the $l_0$-norm ball (our perturbation function) and $l_2$-norm ball are the same because the feature values are within $[0,1]$.
Since RAB targets single-test-input prediction, we do not use Bonferroni correction for \technique as a fair comparison.
We directly cite RAB's results from~\citet{RAB}.
% and denote different configurations as RAB-$\sigma$, where $\sigma$ represents the Gaussian noise level.  
Table~\ref{tab:backdoor_res} shows that on MNIST-01 and CIFAR10-02, \technique achieves similar normal accuracy, but a much higher certified accuracy than RAB for all values of $\assumeradii$~(detailed figures in \Cref{sec: appendix_res}).
\textbf{\technique significantly outperforms RAB against $\featflipone$ on MNIST-01 and CIFAR10-02.}


% \begin{wrapfigure}{R}{0.4\textwidth}
% \vspace{-2em}
%     \include{figs/bd_mnist_contagio}
%   \label{fig:bd_mnist_contagio}
%   \vspace{-2em}
% \end{wrapfigure}
\textbf{Results on MNIST and Contagio.}
Figure~\ref{fig:bd_mnist_contagio} shows the results of \technique on MNIST and Contagio. 
When fixing $\assumeradii$, the certified accuracy for the backdoor attack is much smaller than the certified accuracy for the trigger-less attack~(Figure~\ref{fig:compare_bagging} and Figure~\ref{fig:compare_bagging_full} in \Cref{sec: appendix_res}) because backdoor attacks are strictly stronger than trigger-less attacks.
\technique cannot provide effective certificates for backdoor attacks on the more complex datasets CIFAR10 and EMBER, i.e., the certified radius is almost zero.
\textbf{\technique can provide certificates against backdoor attacks on MNIST and Contagio, while \technique's certificates are not effective for CIFAR10 and EMBER.}

% \aws{again tables can help. what about Ember/Contagio?} 
%  \yh{we don't compare them on Ember and Contagio because I did not run their experiments but directly cite the results.}

\subsection{Computation Cost Analysis}
We discuss the computation cost of \technique on the MNIST dataset and compare to other baselines.

\textbf{Training.} The cost of \technique during training is similar to all the baselines because \technique only adds noise in the training data. 
\technique and other baselines take about 16 hours on a single GPU to train $N=1000$ classifiers on the MNIST dataset.

\textbf{Inference.} At inference time, \technique first evaluates the predictions of $N$ classifiers, and counts how many classifiers have the majority label ($N_1$) and how many have the runner-up label ($N_2$). 
Then, \technique uses a prepared lookup table to query the radius certified by $N_1$ and $N_2$.
The inference time for each example contains the evaluation of $N$ classifiers and an O(1) table lookup. Hence, there is no difference between \technique and other baselines.

\textbf{Preparation.} \technique needs to prepare a table of size O($N^2$) to perform efficient lookup at  inference time. 
The time complexity of preparing each table entry is presented in Sections~\ref{sec:precise_approach} and ~\ref{sec:imprecise}.
On the MNIST dataset, \technique with the relaxation proposed in Section~\ref{sec:imprecise} ($\delta = 10^{-4}$) needs 2 hours to prepare the lookup table on a single core. 
However, the precise \technique proposed in Section~\ref{sec:precise_approach} needs 85 hours to prepare the lookup table. 
Bagging also uses a lookup table that can be built in 16 seconds on MNIST (Bagging only needs to do a binary search for each entry). 
FeatFlip needs approximately 8000 TB of memory to compute its table. Thus, FeatFlip is infeasible to run on the full MNIST dataset. FeatFlip is only evaluated on a subset of the MNIST-17 dataset containing only 100 training examples.
RAB does not need to compute the lookup table because it has a closed-form solution for computing the certified radius.

\textbf{\technique has similar training and inference time compared to other baselines. The relaxation technique in Section~\ref{sec:imprecise} is useful to reduce the preparation time from 85 hours to 2 hours.} 
Even with the relaxation, \technique needs more preparation time than Bagging and RAB. We argue that the preparation of \technique is feasible because it only takes 12.5\% of the time required by training.

==> BagFlip_ A Certified Defense against Data Poisoning/sections/intro.tex <==
\section{Introduction}
Recent works have shown that machine learning models are vulnerable to data-poisoning attacks, where the attackers maliciously modify the training set to influence the prediction of the victim model as they desire.
In a \emph{trigger-less} attack~\cite{triggerless_convpolytope, triggerless_featurecollision, triggerless_SpamFilter, triggerless_SVM, triggerless_bullseyepolytope, triggerless_witchbrew}, the attacker can modify the training set but not the test inputs, while in a \emph{backdoor} attack~\cite{backdoor_hidden, backdoor_labelconsistent, backdoor_latent, backdoor_Malwarepoison, backdoor_targetDL, backdoor_trojan, backdoor_NLP, backdoor_code} the attacker can also modify test inputs.
Effective attack approaches have been proposed for various domains such as image recognition~\cite{badnets}, sentiment analysis~\cite{backdoor_NLP}, and malware detection~\cite{backdoor_Malwarepoison}. 

Consider the malware detection setting.
An attacker can modify the training data by adding a special signature---e.g., a line of code---to a set of benign programs.
The idea is to make the learned model correlate the presence of the signature with benign programs.
Then, the attacker can sneak a piece of malware past the model by including the signature,
fooling the model into thinking it is a benign program.
%
Indeed, it has been shown that if the model is trained on a dataset with only a few poisoned examples, a backdoor signature can be installed in the learned model~\cite{backdoor_Malwarepoison, backdoor_code}.
%
Thus, data-poisoning attacks are of great concern to the safety and security of machine learning models and systems, particularly as training data is gathered from different sources, e.g., via web scraping.

Ideally, a defense against data poisoning should fulfill the following desiderata: (1) Construct \textbf{effective certificates} (proofs) of the defense. (2) Defend against \textbf{both trigger-less and backdoor attacks}. (3) Be \textbf{model-agnostic}.
It is quite challenging to fulfill all three desiderata; indeed, existing techniques are forced to make tradeoffs.
For instance, empirical approaches~\cite{heu_advtrain, heu_featureselect, heu_finetune, heu_gendist, heu_neuralcleanse, heu_robustcovariance, heu_spectral, heu_strip} cannot construct certificates and are likely to be bypassed by new attack approaches~\cite{break_attackdefense, break_backdoorfl, break_sanitization}.
Some certified approaches~\cite{RAB, featureflip}  provide \textit{ineffective} certificates for both trigger-less and backdoor attacks.
Some certified approaches~\cite{bagging, partitioning, framework_def, labelflip, differential, dpa_improve} provide effective certificates for trigger-less attacks but not backdoor attacks. %
Other certification approaches~\cite{certkrNN, decisiontree, prog_decisiontree} are restricted to specific learning algorithms, e.g., decision trees.

This paper proposes \technique, a \textit{model-agnostic certified} approach that uses \emph{randomized smoothing}~\cite{randomizesmoothing, divergences, tightflipbound} to effectively defend against both trigger-less and backdoor attacks~(\Cref{sec:smoothing}). 
\technique uses a novel smoothing distribution that combines \emph{bagging} of the training set and noising of the training data and the test input by randomly \emph{flipping} features and labels.

Although both bagging-based and noise-based approaches have been proposed independently in the literature, combining them makes it challenging to compute the \emph{certified radius}, i.e., the amount of poisoning a learning algorithm can withstand without changing its prediction.

To compute the certified radius precisely, we apply the Neyman--Pearson lemma to the sample space of \technique's smoothing distribution. 
% 
This lemma requires partitioning the outcomes in the sample space into subspaces such that the likelihood ratio in each subspace is a constant.
% 
However, because our sample space is exponential in the number of features, we cannot naively apply the lemma.
% 
To address this problem, we exploit properties of our smoothing distribution to design an efficient algorithm that partitions the sample space into polynomially many subspaces (\Cref{sec:precise_approach}).
Furthermore, we present a \emph{relaxation} of the Neyman–Pearson lemma that further speeds up the computation (\Cref{sec:imprecise}).
Our evaluation against existing approaches shows that \technique is comparable to them or more effective for trigger-less attacks and more effective for backdoor attacks (\Cref{sec: experiment}). 


==> BagFlip_ A Certified Defense against Data Poisoning/sections/legacy.tex <==
\subsubsection{Bound by the KL divergence}
\begin{theorem}
\label{thm:KL_bound}
Consider the binary classification case where $|\mathcal{C}|=2$,
Denote $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'', x)=y^*)$ as $p$, Eq~\ref{eq:certgoal1} holds if 
\begin{align}
    \poisonfeat \poisonins < \dfrac{|D|\log(4p(1-p))}{2k\log(\frac{b}{a})(a-b)},
\end{align}
where $\poisonins$ is the number of the poisoned instances, $\poisonfeat$ is the number of the poisoned features, $k$ is the size of each bag, and $a, b$ are the probability of a featuring remaining the same and being flipped. 
\end{theorem}
% \todo{It seems $T=(a-b)\poisonfeat$, prove that.}

\begin{lemma}
\label{lemma:T}
Define $T$ as
\begin{align}
    T = \sum_{u=0}^d \sum_{v=0}^d |L(u,v;\poisonfeat)| b^u a^{d-u} (v-u)\label{eq:defofT}
\end{align}
and similarly in the Lemma 5 of \citet{tightflipbound}, $|L(u,v;\poisonfeat)|$ is defined as,
\[\sum_{i=\max(0,v-\poisonfeat)}^{\min(u, d-\poisonfeat, \lfloor \frac{u+v-\poisonfeat}{2} \rfloor)} (K-1)^j \binom{\poisonfeat}{j} \binom{\poisonfeat-j}{u-i-j} K^i \binom{d-\poisonfeat}{i},\]
where $j=u+v-2i-\poisonfeat$.
Then 
\[T = (a-b)s\]
\end{lemma}



\textbf{Proof of the Theorem~\ref{thm:KL_bound}.}
\begin{proof}
Denote $D'\sim \mu(D)$ and $D''\sim \mu(\poisoned{D})$, from the theorem in Example 5 of \cite{labelflip}, Eq~\ref{eq:certgoal1} holds if 
\begin{align}
    \KL(D''\|D') < -\frac{1}{2}\log(4p(1-p)) \label{eq:KLproof0}
\end{align}
We now calculate the KL divergence between the distribution generated from the poisoned dataset $\poisoned{D}$ and the distribution generated from the original dataset $D$.
\begin{align}
    &\KL(D''\|D') \nonumber\\
    = &k \KL(D''_1\|D'_1)\label{eq:KLproof1}\\
    = &k \sum_{w=1}^{|D|} \sum_{\bfx} p_{D_1''}(w, \bfx) \log\frac{p_{D_1''}(w, \bfx)}{p_{D_1'}(w, \bfx)}\nonumber\\
    = &k \sum_{w \in \poisoned{I}} \sum_{\bfx} p_{D_1''}(w, \bfx) \log\frac{p_{D_1''}(w, \bfx)}{p_{D_1'}(w, \bfx)}\label{eq:KLproof2}\\
    \le &k\poisonins \sum_{\bfx} \frac{a^d}{|D|}  \left(\frac{b}{a}\right)^{g(\bfx, \poisoned{D}_w)} \log\frac{b}{a} (g(\bfx, \poisoned{D}_w) - g(\bfx, D_w))\nonumber\\
    = & kp_\poisonins a^d \log(\frac{b}{a}) \sum_{\bfx}  \left(\frac{a}{b}\right)^{g(\bfx, \poisoned{D}_w)} (g(\bfx, D_w) - g(\bfx, \poisoned{D}_w))\label{eq:KLproof3}
\end{align}
where $\poisoned{I}$ are the set of poisoned indices, $\KL(D_1'' \| D_1')$ is the KL divergence of the first selected instance.
We have Eq~\ref{eq:KLproof1} because each selected instance is independent. 
We have Eq~\ref{eq:KLproof2} because the $p_{D''_1}(w, \bfx)$ and $p_{D'_1}(w, \bfx)$ only differs when the $w$th instance is poisoned.

The attacker can modify $\poisoned{D}_w$ to maximize Eq~\ref{eq:KLproof3}. And the Lemma 4 in \citet{tightflipbound} states that the maximal value is achieved when $\poisoned{D}_w$ has exact $\poisonfeat$ features flipped to another value. Because the independence of the features, it does not matter which of them are flipped.

Now suppose the first $\poisonfeat$ features are flipped in $\poisoned{D}_w$, we then need to compute Eq~\ref{eq:KLproof3}. 
If we denote $g(\bfx, \poisoned{D}_w)$ as $u$ and $g(\bfx, D_w)$ as $v$, and we count the size of the set $L(u,v;\poisonfeat)=\{\bfx \mid g(\bfx, \poisoned{D}_w) = u, g(\bfx, D_w) = v\}$, then we can compute Eq~\ref{eq:KLproof3} as
\begin{align*}
   kp_\poisonins a^d \log(\frac{a}{b}) \sum_{u=0}^d \sum_{v=0}^d |L(u,v;\poisonfeat)| \left(\frac{b}{a}\right)^{u}(v-u) 
\end{align*}
Let $T$ be defined as in Eq~\ref{eq:defofT}, we then have
\begin{align}
    \KL(D'' \| D') = kp_\poisonins \log(\frac{a}{b})T \label{eq:KLproof4}
\end{align}
Combine Eq~\ref{eq:KLproof0}, Eq~\ref{eq:KLproof4}, and Lemma~\ref{lemma:T}, we have 
\begin{align*}
    kp_\poisonins \log(\frac{a}{b})(a-b)\poisonfeat <& -\frac{1}{2}\log(4p(1-p))\\
    \poisonins \poisonfeat <& \dfrac{|D|\log(4p(1-p))}{2k\log(\frac{b}{a})(a-b)}
\end{align*}
\end{proof}

\textbf{Proof of the Lemma~\ref{lemma:T}.}
\begin{proof}
Notice that the value of $T$ does not defend on the feature dimension $d$. 
Thus, we prove the lemma by induction on $d$.
We further denote the value of $T$ under the feature dimension $d$ as $T_d$.

\textbf{Base case.} Because $0 \le s \le d$, when $d = 0$, it is easy to see $T_0 = s(a-b) = 0$.

\textbf{Induction case.} 
We first prove $T_{d+1}=s(a-b)$ under a special case, where $s = d+1$, given the inductive hypothesis $T_d = s(a-b)$ for all $s = d$. 

By definition
\begin{align}
    T_{d+1} = \sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u,v;\poisonfeat;d+1)| b^u a^{d+1-u} (v-u),\label{eq:lemmaT0}
\end{align}
where we denote $L(u,v;\poisonfeat)$ as $L(u,v;\poisonfeat;d+1)$ when feature dimension is $d+1$.

By the definition of $L(u,v;\poisonfeat)$, we have the following equation when $0 \le s \le d$
\begin{align}
    |L(u,v;d+1;d+1)| = (K-1)|L(u-1,v-1;d;d)| +\nonumber\\ |L(u-1,v;d;d)| + |L(u,v-1;d;d)|\label{eq:lemmaT4}
\end{align}
and 
\begin{align}
    \sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^u a^{d-u} = 1\label{eq:lemmaT8}
\end{align}
Plug Eq~\ref{eq:lemmaT4} into Eq~\ref{eq:lemmaT0}, we have the following equations when $s = d+1$,
\begin{align}
    T_{d+1} = &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} (K-1)|L(u-1,v-1;d;d)|b^u a^{d+1-u} (v-u) + \nonumber\\
    &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u-1,v;d;d)| b^u a^{d+1-u}  (v-u)+\nonumber\\
    &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u,v-1;d;d)| b^u a^{d+1-u} (v-u)\nonumber\\
    = &b(K-1)\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)|b^u a^{d-u} (v-u) + \label{eq:lemmaT5}\\
    &b\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^{u} a^{d-u} (v-u-1)+\label{eq:lemmaT6}\\
    &a\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^{u} a^{d-u} (v-u+1)\label{eq:lemmaT7}\\
    = & \sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^{u} a^{d-u} [(v-u) + (a-b)] \nonumber\\
    = &d(a-b) + (a-b)\label{eq:lemmaT9}\\
    = &\poisonfeat(a-b)\nonumber
\end{align}
We have Eq~\ref{eq:lemmaT4}, Eq~\ref{eq:lemmaT5} and Eq~\ref{eq:lemmaT6} because $L(u,v;\poisonfeat,d)=0$ when $u>d$, $v>d$, $u<0$ , or $v<0$.
We have Eq~\ref{eq:lemmaT9} by plugging in Eq~\ref{eq:lemmaT8}.

Next, we are going to show that $T_{d+1} = s(a-b)$ for all $0 \le s \le d$, given the inductive hypothesis $T_d = s(a-b)$ for all $0 \le s \le d$. 

By the definition of $L(u,v;\poisonfeat)$, we have the following equations when $0 \le s \le d$
\begin{align}
    |L(u,v;\poisonfeat;d+1)| = |L(u,v;\poisonfeat;d)| + K|L(u-1,v-1;\poisonfeat;d)|\label{eq:lemmaT1}
\end{align}
Plug Eq~\ref{eq:lemmaT1} into Eq~\ref{eq:lemmaT0}, for all $0 \le s \le d$, we have
\begin{align}
    T_{d+1} = &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u,v;\poisonfeat;d)|b^u a^{d+1-u} (v-u) + \nonumber\\
    &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} K|L(u-1,v-1;\poisonfeat;d)| b^u a^{d+1-u} (v-u)\nonumber\\
    = &a\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;\poisonfeat;d)|b^u a^{d-u} (v-u) + \label{eq:lemmaT2}\\
    &bK\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;\poisonfeat;d)| b^{u} a^{d-u} (v-u)\label{eq:lemmaT3}\\
    = & as(a-b) + bKs(a-b) \nonumber\\
    = &s(a-b)\nonumber
\end{align}
We have Eq~\ref{eq:lemmaT2} and Eq~\ref{eq:lemmaT3} because $L(u,v;\poisonfeat,d)=0$ when $u>d$, $v>d$, $u<0$ , or $v<0$.


\end{proof}

% The following bound is quite loose, but it makes easier to understand the relation between parameters. 
% \begin{corollary}
% \label{coro:KL}
% Eq~\ref{eq:certgoal1} holds if 
% \begin{align}
%     \poisonfeat < \dfrac{\log(4p(1-p))}{2k\log(\frac{b}{a})p_\poisonins}
% \end{align}
% \end{corollary}
% We get the above corollary because we can derive an upper bound of $T$ as $\poisonfeat$.


% \begin{proof}
% Notice that an upper bound of Eq~\ref{eq:KLproof3} is 
% \begin{align}
%     &kp_\poisonins a^d \log(\frac{b}{a}) \sum_{\bfx} \left(\frac{b}{a}\right)^{g(\bfx, \poisoned{D}_w)}(-\poisonfeat) \nonumber\\
%     =& kp_\poisonins a^d \log(\frac{a}{b})\poisonfeat \sum_{\bfx}  \left(\frac{b}{a}\right)^{g(\bfx, \poisoned{D}_w)}\nonumber\\
%     =& kp_\poisonins a^d \log(\frac{a}{b})\poisonfeat \sum_{i=0}^d \binom{d}{i} K^i \left(\frac{b}{a}\right)^i \nonumber \\
%     =& kp_\poisonins a^d \log(\frac{a}{b})\poisonfeat (1 + \frac{Kb}{a})^d \nonumber\\
%     =& kp_\poisonins \log(\frac{a}{b})\poisonfeat, \label{eq:coro1proof0}
% \end{align}
% because the attacker can flip at most $\poisonfeat$ features, then $g(\bfx, \poisoned{D}_w)-g(\bfx, D_w)$ is lower bounded by $-\poisonfeat$ (notice that $\log(\frac{b}{a})$ is negative).
% Combine Eq~\ref{eq:KLproof0} and Eq~\ref{eq:coro1proof0}, we have 
% \begin{align*}
%     kp_\poisonins\log(\frac{a}{b})\poisonfeat <& -\frac{1}{2}\log(4p(1-p))\\
%     \poisonfeat <& \dfrac{\log(4p(1-p))}{2k\log(\frac{b}{a})p_r}
% \end{align*}
% \end{proof}

\begin{corollary}
\label{coro:KL_cert}
From Theorem~\ref{thm:KL_bound}, we can compute the certified radius $R_{cert}(\poisonins)$ as
\begin{align}
    R_{cert}(\poisonins) = \min(d, \lceil \dfrac{|D|\log(4p(1-p))}{2k\log(\frac{1-a}{aK})\frac{a(K+1)-1}{K}\poisonins} \rceil - 1) \label{eq:cert_radius}
\end{align}
\end{corollary}

\begin{remark}
From Eq~\ref{eq:cert_radius}, we know that the certified radius becomes larger when the classifiers accuracy $p$ is larger, the number of instances in the bag $k$ is smaller, the probability of remaining the same $a$ is smaller, the number of categories of each feature $K$ is smaller, or the number of poisoned instances $\poisonins$ is smaller.

However, there is a trade-off between $p$ and $a$ because the more noise is added to the training set, the lower the performance of each classifier gets. 
There is also a trade-off between $p$ and $k$ because the less instances is in the bag, the lower the performance of each classifier gets.
\end{remark}

% \begin{remark}
% Note that, if the features are not categorized, the category number $K$ can still be upper bounded by $|D|$ because each feature has at most $|D|$ different values in the training set, as we can randomly flip each feature to an existing features in the bag. Then the certified radius $R_{cert}(\poisonins)$ can be computed as
% \begin{align*}
%     R_{cert}(\poisonins) = \max(d, \lceil \dfrac{\log(4p(1-p))|D|^2}{2k\log(\frac{1-a}{a|D|})\poisonins} \rceil - 1) 
% \end{align*}
% \end{remark}

\subsubsection{Combine the Neyman-Pearson Lemma and the KL divergence}
As in the previous sections, we show an efficient relaxation of the bound computed by the Neyman-Pearson Lemma. 
The relaxation simply ignores all subspaces $\mathcal{L}^{l+1}(\bfc, \bfu, \bfv),\mathcal{L}^{l+2}(\bfc, \bfu, \bfv),\ldots, \mathcal{L}^k(\bfc, \bfu, \bfv)$.
However, we can get a tighter bound by applying the KL divergence bound to the ignored subspaces. 
\begin{lemma}
The KL divergence between $\mu(\poisoned{D})$ and $\mu(D)$ on the subspace $\bigcup_{i=l+1}^k \mathcal{L}^i(\bfc, \bfu, \bfv)$ is 
\[(kp_\poisonins - lp_\poisonins + l)\log(\frac{a}{b})T\]
\end{lemma}

\begin{lemma}
\label{lemma:extendedKL}
Consider the binary classification case, denoting $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'', x)=y^*)$ as $p$, 
\begin{align*}
    (1-\lambda)\underset{D'\sim \mu(D)}{\PP}(f(D', x)=y^*) > \lambda\underset{D'\sim \mu(D)}{\PP}(f(D', x)=y)
\end{align*}
holds for all $y \neq y^*$ if 
\begin{align*}
    \mathrm{KL}(D''\| D') < \log(\frac{(1-\lambda)p}{\lambda(1-p)})(1-\lambda) - \log(\frac{p}{\lambda})
\end{align*}
Specifically, if we consider the subspace $\bigcup_{i=l+1}^k \mathcal{L}^i(\bfc, \bfu, \bfv)$, then
\begin{align}
    (kp_\poisonins - lp_\poisonins + l)\log(\frac{a}{b})T < \log(\frac{(1-\lambda)p}{\lambda(1-p)})(1-\lambda) - \log(\frac{p}{\lambda})\label{eq:generalKL}
\end{align}
\end{lemma}

\begin{remark}
Lemma~\ref{lemma:extendedKL} is a more general KL divergence bound and \citet{divergences} provided a special case when $\lambda=\frac{1}{2}$, which is used in Theorem~\ref{thm:KL_bound}. 
We need the general version for the following theorem.
\end{remark}

\begin{theorem}
Consider the binary classification case, denoting $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'', x)=y^*)$ as $p$ and choosing $l$ for computing the feasible Neyman-Pearson bound, Eq~\ref{eq:certgoal1} holds if for all $\gamma \in [0, 1 - F(l;k,p_\poisonins)]$,
\begin{align}
    \mathrm{NP_{bound}}(\frac{p-\gamma}{F(l;k,p_\poisonins)})F(l;k,p_\poisonins) +\nonumber\\ \mathrm{KL_{bound}}(\frac{\gamma}{1 - F(l;k,p_\poisonins)})(1-F(l;k,p_\poisonins)) \ge \frac{1}{2},
\end{align}
where $\mathrm{NP_{bound}}(z)$ computes the lower bound $lb_l$ when $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'',x)=y^*)$ is set to $z$ and $\mathrm{KL_{bound}}(z)$ computes the largest $\lambda$ satisfying Eq~\ref{eq:generalKL} when $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'',x)=y^*)$ is set to $z$.
\end{theorem}

\subsection{Compare to the bagging and the feature-flipping approach}
We compare the certified radius computed from Corollary~\ref{coro:KL_cert} to the certified radius computed from the bagging approach~\cite{bagging} and the feature-flipping approach~\cite{featureflip}.

We look at a realistic dataset MNIST 1/7 dataset ($d=28*28+1=785$, i.e., we also consider label-flipping attack) that just includes digits 1 and 7. This subset includes 13,007 training examples ($|D|=13007$) and 2,163 testing examples. 
In \citet{bagging}, they choose the bagging size $k=50$ and the probability $a=0.7$. 
Also, we assume that the classifier performance $p=0.8$ because the task is relatively easy. And we will further justify this aspect in the experiment section.

From Corollary 1 in~\citet{bagging}, we can compute $R_{bag}=92$.
From the experiment section in~\citet{featureflip}, we use an upper bound of $R_{ff}=3d=2355$ for comparison.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/sim_bounds}
    \caption{$R_{cert}$ computed by three approaches.}
    \label{fig:sim_bounds}
\end{figure}

\todo{Wrong!} Figure~\ref{fig:sim_bounds} shows the results of $R_{cert}$ computed by three approaches. 
Our approach can certify up to $\poisonins=1135$ poisoned instances modified in the training set assuming the attacker can flip all features in the instance (i.e., $R_{cert}(1135)=d$). And our approach can certify up to $\poisonfeat=68$ features being flipped assuming the attacker can modify all instances in the training set (i.e., $R_{cert}(|D|)=68$).

\begin{remark}
Notice that this result is based on the assumption that we can achieve a classifier performance $p=0.8$, given $k=50$ and $a=0.7$. 
However, our approach may require larger $k$ to mitigate the effect of noise and may require larger $a$ to mitigate the insufficient bagging size. 

Also, the comparison is not fair for~\citet{bagging} because the bagging approach does not assume all features are categorized. 
\end{remark}

\subsection{Certified defense of data poisoning and evasion attack}


==> BagFlip_ A Certified Defense against Data Poisoning/sections/problemdef.tex <==
\section{Problem Definition}
\label{sec: prob_def}

We take a holistic view of training and inference as a single deterministic algorithm $\alg$.
Given a dataset $D = \{(\bfx_1, y_1), \ldots, (\bfx_n, y_n)\}$
% we write $\model{D}$ to denote an algorithm $\alg$ training on $D$.
% 
and a (test) input $\bfxtest$, we write $\modelpred{D}{\bfxtest}$ to denote the prediction of algorithm $\alg$ on the input $\bfxtest$ after being trained on dataset $D$.

% \yh{modified, please check.}
We are interested in certifying that the algorithm will still behave ``well'' after training on a tampered dataset.
%
Before describing what ``well'' means, to define our problem we need to assume a \emph{perturbation space}---i.e., what possible changes the attacker could make to the dataset.
% 
Given a pair $(\bfx, y)$, we write $\perturb(\bfx, y)$ to denote the set of perturbed examples that an attacker can transform the example $(\bfx, y)$ into. 
% 
Given a dataset $D$ and a \textit{radius} $\poisonins\geq 0$, we define the \textit{perturbation space} as the set of datasets that can be obtained by modifying up to $\poisonins$ examples in $D$ using the perturbation $\perturb$:
\[
\poisonset{\perturb} = \left\{\{(\poisoned{\bfx}_i, \poisoned{y}_i)\}_i ~\bigg|~ \forall i.\ (\poisoned{\bfx}_i, \poisoned{y}_i) \in \perturb(\bfx_i, y_i),\ \sum_{i=1}^n \mathds{1}_{(\poisoned{\bfx}_i, \poisoned{y}_i) \neq (\bfx_i,y_i)} \le r\right\}
\]

\textbf{Threat models.}
We consider two attacks: one where an attacker can perturb only the training set (a \emph{trigger-less} attack) and one where the attacker can perturb both the training set and the test input (a \emph{backdoor} attack). We assume a backdoor attack scenario where test input perturbation is the same as training one.
If these two perturbation spaces can perturb examples differently, we can always over-approximate them by their union.
% 
In the following definitions, we assume that we are given a perturbation space $\perturb$, a radius $\poisonins\geq 0$, and a benign training dataset $D$ and test input $\bfx$.


% , a dataset $\poisoned{D}$ (which we assume is the result of the attacker perturbation).
% 
% We also assume the existence of an \textit{unknown} benign dataset $D$ from which $\poisoned{D}$ could have been obtained. 

We say that algorithm $\alg$ is robust to a \textbf{trigger-less attack} on the test input $\bfxtest$ if $\alg$  yields the same prediction on the input $\bfxtest$ when trained on any perturbed dataset $\poisoned{D}$ and the benign dataset $D$. Formally,
\begin{align}
    \forall \poisoned{D} \in \poisonset{\perturb}.\ \modelpred{\poisoned{D}}{\bfxtest} = \modelpred{D}{\bfxtest}\label{eq:trigger_less_goal}
\end{align}

We say that algorithm $\alg$ is robust to a \textbf{backdoor attack} on the test input $\bfxtest$ 
if the algorithm trained on any perturbed dataset $\poisoned{D}$ produces the prediction $\modelpred{D}{\bfxtest}$ 
on any perturbed input $\poisoned{\bfxtest}$. 
Let $\perturb(\bfxtest, \ytest)_1$ denote the projection of the perturbation space $\perturb(\bfxtest, \ytest)$ onto the feature space (the attack can only backdoor features of the test input).
Robustness to a backdoor attack is defined as
\begin{align}
     \forall \poisoned{D} \in \poisonset{\perturb},\ \poisoned{\bfxtest} \in \perturb(\bfxtest, \ytest)_1.\ \modelpred{\poisoned{D}}{\poisoned{\bfxtest}} = \modelpred{D}{\bfxtest}\label{eq:goal}
\end{align}

Given a large enough radius $r$, an attacker can always change enough examples and succeed at breaking robustness for either kind of attack. 
% 
Therefore, we will focus on computing the maximal radius $r$, for which we can prove that Eq~\ref{eq:trigger_less_goal}~and~\ref{eq:goal} hold for a given  perturbation function $\perturb$.
% 
We refer to this quantity as the \textit{certified radius}.
% 
It is infeasible to prove Eq~\ref{eq:trigger_less_goal}~and~\ref{eq:goal} by enumerating all possible $\poisoned{D}$ because $\poisonset{\perturb}$ can be ridiculously large, e.g., $|\poisonset{\perturb}| > 10^{30}$ when $|D|=1000$ and $\poisonins=10$.

\textbf{Defining the perturbation function.}
We have not yet specified the perturbation function $\perturb$, i.e., how the attacker can modify examples.
% 
In this paper, we focus on the following perturbation spaces.

Given a bound $\poisonfeat \geq 0$, a \textbf{feature-and-label-flipping perturbation}, $\featfliplabelflip$, allows the attacker to modify the values of up to $\poisonfeat$ features and the label in an example $(\bfx, y)$, where $\bfx \in [K]^d$ (i.e., $\bfx$ is a $d$-dimensional feature vector with each dimension having $\{0,1,\ldots, K\}$ categories). Formally,
    \begin{align*}
            \featfliplabelflip(\bfx, y) = \{(\poisoned{\bfx}, y')\mid \|\bfx - \poisoned{\bfx}\|_0 + \mathds{1}_{y\neq y'} \le \poisonfeat\}, 
    \end{align*}
There are two special cases of $\featfliplabelflip$, a \textbf{feature-flipping perturbation} $\featflip$ and a \textbf{label-flipping perturbation} $\labelflip$.
Given a bound $\poisonfeat \geq 0$, $\featflip$ allows the attacker to modify the values of up to $\poisonfeat$ features in the input $\bfx$ but not the label.
$\labelflip$ only allows the attacker to modify the label of a training example. Note that $\labelflip$ cannot modify the test input's features, so it can only be used in trigger-less attacks.

\begin{example}
\label{exp: perturbation}
If $D$ is a binary-classification image dataset, where each pixel is either black or white, then the perturbation function $\featflipone$ assumes the attacker can modify up to one pixel per image. 
\end{example}

    % \[\featflip(\bfx, y) = \{(\poisoned{\bfx}, y)\mid \|\bfx - \poisoned{\bfx}\|_0 \le \poisonfeat\},\quad  \mathrm{proj}_{\bfx}(\featflip(\bfx, y)) = \{\poisoned{\bfx} \mid \|\bfx - \poisoned{\bfx}\|_0 \le \poisonfeat\},\]
    
% \aws{check this para}
% \paragraph{Certified guarantees}
The goal of this paper is to design a certifiable algorithm that can defend against trigger-less and backdoor attacks (Section~\ref{sec:smoothing}) by computing the certified radius (Sections~\ref{sec:precise_approach}~and~\ref{sec:imprecise}).
Given a benign dataset $D$, our algorithm certifies that an attacker can perturb $D$ by some amount (the certified radius) 
without changing the prediction.
Symmetrically, if we suspect that $D$ is poisoned, our algorithm certifies that even if an attacker had not poisoned $D$ by up to the certified radius, the prediction would have been the same.
The two views are equivalent, and we use the former in the paper.

==> BagFlip_ A Certified Defense against Data Poisoning/sections/relatedwork.tex <==
\section{Related Work}
\label{sec: related_work}
% \loris{remove this paragraph, it's a copy paste of the intro. Move refs to intro if some are different.}
% Machine learning models are vulnerable to data poisoning, such as trigger-less attacks~\cite{triggerless_convpolytope, triggerless_featurecollision, triggerless_SpamFilter, triggerless_SVM, triggerless_bullseyepolytope, triggerless_witchbrew} and backdoor attacks~\cite{backdoor_hidden, backdoor_labelconsistent, backdoor_latent, backdoor_Malwarepoison, backdoor_targetDL, backdoor_trojan, backdoor_NLP, backdoor_code}.
% Although many heuristic defense approaches~\cite{heu_advtrain, heu_featureselect, heu_finetune, heu_gendist, heu_neuralcleanse, heu_robustcovariance, heu_spectral, heu_strip} have been proposed, attacks can often break these heuristic approaches~\cite{break_attackdefense, break_backdoorfl, break_sanitization}. Therefore, \textit{certified defenses} are crucial for data poisoning attacks. 

% The following paragraph summarizes how our work differs from the aforementioned ones.
Our \textit{model-agnostic} approach \technique uses randomized smoothing to compute \textit{effective certificates} for \textit{both} trigger-less and backdoor attacks.
\technique focuses on feature-and-label-flipping perturbation functions that modify training examples and test inputs.
We discuss how existing approaches differ.

Some model-agnostic certified approaches can defend against both trigger-less and backdoor attacks but cannot construct effective certificates.
\citet{featureflip, RAB} defended feature-flipping poisoning attacks and $l_2$-norm poisoning attacks, respectively.
However, their certificates are practically ineffective due to the curse of dimensionality~\cite{curse}.

Some model-agnostic certified approaches construct effective certificates but cannot defend against backdoor attacks.
\citet{bagging} proposed to defend against \textit{general} trigger-less attacks, i.e., the attackers can add/delete/modify examples in the training dataset, by bootstrap aggregating (bagging).
\citet{framework_def} extended bagging by designing other selection strategies, e.g., selecting without replacement and with a fixed probability.
\citet{labelflip} defended against label-flipping attacks and instantiated their framework on linear classifiers.
Differential privacy~\cite{differential} can also provide probabilistic certificates for trigger-less attacks, but it cannot handle backdoor attacks, and its certificates are ineffective.
\citet{partitioning} proposed a deterministic partition aggregation~(DPA) to defend against general trigger-less attacks by partitioning the training dataset using a secret hash function. 
\citet{dpa_improve} further improved DPA by introducing a spread stage.

Other certified approaches construct effective certificates but are not model-agnostic.
\citet{certkrNN} provided deterministic certificates \textit{only} for nearest neighborhood classifiers~(kNN/rNN), but for both trigger-less and backdoor attacks.
\citet{prog_decisiontree, decisiontree} provided deterministic certificates \textit{only} for decision trees but against general trigger-less attacks.

% Although deterministic approaches for specific machine learning models can potentially provide more effective certificates, they are not model-agnostic compared to \technique.


==> BagFlip_ A Certified Defense against Data Poisoning/sections/theorem.tex <==

\section{A Precise Approach to Computing the Certified Radius}
\label{sec:precise_approach}
% \yh{decide which symbol for $\outcome$.}

In this section, we show how to compute the certified radius of the smoothed algorithm $\salg$ given a dataset $D$, a test input $\bfxtest$, and a perturbation function $\perturb$.
We focus on binary classification and provide the multi-class case in \cref{sec: lemma_multi_class}.

Suppose that we have computed the prediction $\firsty=\smodelpred{D}{\bfxtest}$.
% 
We want to show how many examples we can perturb in $D$ to obtain any other $\poisoned{D}$ so the prediction remains $\firsty$.
Specifically, we want to find the largest possible radius $\poisonins$  
such that 
\begin{align}
    \forall \poisoned{D} \in \poisonset{\perturb},\ \poisoned{\bfxtest} \in \perturb(\bfxtest, \ytest)_1.\ \underset{\sample{D}, \sample{\bfxtest} \sim \mu(\poisoned{D},\poisoned{\bfxtest})}{\PP}(\modelpred{\sample{D}}{\sample{\bfxtest}}=\firsty) > 0.5 \label{eq:certgoal1}
\end{align}
We first show how to \textit{certify} that Eq~\ref{eq:certgoal1} holds for a given $\poisonins$ and then rely on binary search to compute the largest $\poisonins$, i.e., the certified radius.\footnote{It is difficult to get a closed-form solution of the certified radius (as done in~\cite{bagging, RAB}) in our setting because the distribution of \technique is complicated. We rely on binary search as it is also done in \citet{featureflip, tightflipbound}. \Cref{sec: kl_bound} shows a \textit{loose}  closed-form bound on the certified radius by KL-divergence~\cite{divergences}.}
In \Cref{sec: lemma}, we present the Neyman--Pearson lemma to certify Eq~\ref{eq:certgoal1} as it is a common practice in randomized smoothing. 
In \Cref{sec: featflip}, we show how to compute the certified radius for the distribution $\selectflip$ and the perturbation functions $\featflip, \featfliplabelflip$, and $\labelflip$.

\subsection{The Neyman--Pearson Lemma}
\label{sec: lemma}

Hereinafter, we simplify the notation and use $\outcome$ to denote the pair $(\sample{D},\sample{\bfxtest})$ and $\modelpredo{\outcome}$ to denote the prediction of the algorithm training and evaluating on $\outcome$.
We further simplify the distribution $\mu(D,\bfxtest)$ as $\cleandist$ and the distribution $\mu(\poisoned{D},\poisoned{\bfxtest})$ as $\poisondist$.
We define the performance of the smoothed algorithm $\salg$ on dataset $D$, i.e., the probability of predicting $\firsty$, as $\firstp = \PP_{\outcome \sim \cleandist}(\modelpredo{\outcome}=\firsty)$.

The challenge of certifying Eq~\ref{eq:certgoal1} is that we cannot directly estimate the performance of the smoothed algorithm on the perturbed data, i.e., $\PP_{\outcome \sim \poisondist}(\modelpredo{\outcome}=\firsty)$, because $\poisondist$ is universally quantified. 
To address this problem, we use the Neyman--Pearson lemma to find a lower bound $\lb$ for $\PP_{\outcome \sim \poisondist}(\modelpredo{\outcome}=\firsty)$.
We do so by constructing a worst-case algorithm $\sualg$ and distribution $\poisondist$.
Note that we add the superscript $?$ to denote a worst-case algorithm.
Specifically, we minimize $\PP_{\outcome \sim \poisondist}(\umodelpredo{\outcome}=\firsty)$ while maintaining the algorithm's performance on $\cleandist$, i.e., keeping $\PP_{\outcome \sim \cleandist}(\umodelpredo{\outcome}=\firsty) = \firstp$.
We use $\mathcal{A}$ to denote the set of all possible algorithms.
% and, as stated earlier, use $\firsty$ and $\firstp$ to denote the top prediction and the probability of making that top prediction on algorithm $\salg$, respectively.
We formalize the computation of the lower bound $\lb$ as the following constrained minimization objective:  
%
\begin{small}
\begin{align}
    \lb \triangleq \min_{\sualg\in \mathcal{A}} \underset{\outcome \sim \poisondist}{\PP}(\umodelpredo{\outcome}=\firsty)\label{eq:lbub}
    \ \ \ \ s.t.&\ \underset{\outcome \sim \cleandist}{\PP}(\umodelpredo{\outcome}=\firsty)=\firstp
    \text{ and }  \poisoned{D} \in \poisonset{\perturb}, \poisoned{\bfxtest} \in \perturb(\bfxtest, \ytest)_1 
\end{align}
\end{small}%
%
It is easy to see that $\lb$ is the lower bound of $\PP_{\outcome \sim \poisondist}(\modelpredo{\outcome}=\firsty)$ in Eq.~\ref{eq:certgoal1} because $\salg \in \mathcal{A}$ and $\salg$ satisfies the minimization constraint.
Thus, $\lb > 0.5$ implies the correctness of Eq.~\ref{eq:certgoal1}.

We show how to construct $\sualg$ and $\poisondist$ greedily.
For each outcome $\outcome=(\sample{D},\sample{\bfxtest})$ in the sample space $\Omega$---i.e., the set of all possible sampled datasets  and test inputs---we define the likelihood ratio of $\outcome$ as $\eta(\outcome) = p_{\cleandist}(\outcome) / p_{\poisondist}(\outcome)$, where $p_{\cleandist}$ and $p_{\poisondist}$ are the PMFs of $\cleandist$ and $\poisondist$, respectively.

The key idea is as follows: We partition $\Omega$ into finitely many disjoint subspaces $\subspace_1, \ldots, \subspace_m$ such that the likelihood ratio in each subspace $\subspace_i$ is some constant $\eta_i \in [0,\infty]$, i.e., $\forall \outcome \in \subspace_i. \eta(\outcome) = \eta_i$.
We can sort and reorder the subspaces by likelihood ratios such that $\eta_1 \ge \ldots \ge \eta_m$. 
% \loris{explain why this is useful}. 
% One way to partition $\Omega$ is to let each subspace contain a singleton outcome. However, the number of possible outcomes can be too large for computation. Therefore, we need to reduce the number of subspaces by grouping outcomes with the same likelihood ratios into the same subspace.
We denote the probability mass of $\cleandist$ on subspace $\subspace_i$ as $\cleandistmass{\subspace_i}$.

\begin{example}
\label{exp: merge}
Suppose $\cleandistmass{\outcome_1} {=} \frac{4}{10}, \poisondistmass{\outcome_1} {=} \frac{4}{10}, \cleandistmass{\outcome_2} {=} \frac{1}{10}, \poisondistmass{\outcome_2} {=} \frac{1}{10}, \cleandistmass{\outcome_3} {=} \frac{4}{10}, \poisondistmass{\outcome_3} {=} \frac{1}{10}$, $\cleandistmass{\outcome_4} {=} \frac{1}{10}, \poisondistmass{\outcome_4} {=} \frac{4}{10}$.
We can partition $\outcome_1$ and $\outcome_2$ into one subspace $\subspace$ because $\eta(\outcome_1) {=} \eta(\outcome_2) {=} 1$. 
% Notice that $\eta(\subspace) = 1$, as well.
% \aws{$\eta(\subspace)$ is never defined / perhaps remove last line}
\end{example}

The construction of the $\sualg$ that minimizes Eq.~\ref{eq:lbub} is a greedy process, which iteratively assigns $\umodelpredo{\outcome} = \firsty$ for $\subspace_1, \subspace_2, \ldots$ until the budget $\firstp$ is met.
The worst-case $\poisondist$ can also be constructed greedily by maximizing the top-most likelihood ratios, and we can prove that the worst-case happens when the difference between $\cleandist$ and $\poisondist$ is maximized, i.e., $\poisoned{D}$ and $\poisoned{\bfx}$ are maximally perturbed.
The following theorem adapts the Neyman--Pearson lemma to our setting.

\begin{theorem}[Neyman--Pearson Lemma for $\featfliplabelflip, \featflip, \labelflip$]
\label{thm:np_bound}
Let $\poisoned{D}$ and $\poisoned{\bfx}$ be a maximally perturbed dataset and test input, i.e., $|\poisoned{D} \setminus D|=\poisonins$, $\dis{\poisoned{\bfxtest}}{\bfxtest} = \poisonfeat$, and $\dis{\poisoned{\bfxtest}_i}{\bfxtest_i} + \mathds{1}_{\poisoned{y}_i \neq y_i} = \poisonfeat$, for each perturbed example $(\poisoned{\bfxtest}_i, \poisoned{y}_i)$ in $\poisoned{D}$.
Let $i_\lb \triangleq \mathrm{argmin}_{{i \in [1,m]}} \sum_{j=1}^i \cleandistmass{\subspace_j} \ge \firstp$. 
Then, 
$\lb = \sum_{j=1}^{i_\lb - 1} \poisondistmass{\subspace_j} + \left(\firstp - \sum_{j=1}^{i_\lb - 1} \cleandistmass{\subspace_j}\right)/\eta_{i_\lb}$.
\end{theorem}

% \aws{i don't see the reason for the first sentence. Existence of "more" algorithms in the set just means you'll get a worse lower bound}
% Note that we relax the algorithm set $\mathcal{A}$ to include probabilistic algorithms, as the minimizer $\sualg$ in the above theorem is probabilistic in $\subspace_{i_\lb}$, i.e., $\PP(\umodelpredo{\outcome} = \firsty)$ is a probability in $[0,1]$. However, $\lb$ will still be a lower bound because $\salg \in \mathcal{A}$.
We say that $\lb$ is \emph{tight} due to the existence of the minimizer $\sualg$ and $\poisondist$ (see  \Cref{sec: lemma_multi_class}).

\begin{example}
\label{exp: lemma}
Following \Cref{exp: merge}, suppose $\Omega = \{\outcome_1, \ldots, \outcome_4\}$ and we partition it into $\subspace_1 = \{\outcome_3\}, \subspace_2 = \{\outcome_1, \outcome_2\}$, $\subspace_3 = \{\outcome_4\}$, and $\eta_1 = 4, \eta_2 = 1, \eta_3 = 0.25$.
Let $\firstp=0.95$, then we have $i_\lb = 3$ and $\lb = 0.1 + 0.5 + (0.95-0.4-0.5) / 0.25 = 0.8$.
\end{example}

\subsection{Computing the Certified Radius of \technique}
\label{sec: featflip}
% \input{tables/symbols}
Computing the certified radius boils down to computing $\lb$ in Eq~\ref{eq:lbub} using Theorem~\ref{thm:np_bound}.
To compute $\lb$ for \technique, we address the following two challenges: 
1) The argmin of computing $i_\lb$ and the summation of $\lb$ in Theorem~\ref{thm:np_bound} depend on the number of subspaces $\subspace_j$'s.
    We design a \textbf{partition strategy} that partitions $\Omega$ into a polynomial number of subspaces~($O(k^2d)$).
    Recall that $k$ is the size of the bag sampled from $D$
    and $d$ is the number of features.
2) In Theorem~\ref{thm:np_bound}, $\lb$ depends on $\cleandistmass{\subspace_j}$, which according to its definition~(Eq~\ref{eq:prd'}) can be computed in exponential time~($O(kd^{2k})$).
    We propose an \textbf{efficient algorithm} that computes these two quantities in polynomial time~($O(d^3+k^2d^2)$).
    
We first show how to address these challenges for $\featflip$ and then show how to handle $\featfliplabelflip$ and $\labelflip$.

\textbf{Partition strategy.}
We partition the large sample space $\Omega$ into disjoint subspaces $\subspace_{c,t}$ that depend on $c$, the number of perturbed examples in the sampled dataset, and $t$, the number of features the clean data and the perturbed data differ on with respect to the sampled data.
Intuitively, $c$ takes care of the bagging distribution and $t$ takes care of the feature-flipping distribution.
Formally, 
\begin{small}
\begin{align}
    \subspace_{c,t} = \{&(\{(\bfx_{w_i}', y_{w_i})\}_i, \bfx')\mid \nonumber\\
    &\sum_{i=1}^k \mathds{1}_{\bfx_{w_i} \neq \poisoned{\bfx}_{w_i}}=c ,\label{eq:Ldef1} \\
    &\underbrace{\left(\sum_{i=1}^k \dis{\bfx_{w_i}'}{\bfx_{w_i}} + \dis{\bfx'}{\bfxtest}\right)}_{\diffu} - \underbrace{\left(\sum_{i=1}^k \dis{\bfx_{w_i}'}{\poisoned{\bfx}_{w_i}} + \dis{\bfx'}{\poisoned{\bfxtest}}\right)}_{\diffv} = t\}\label{eq:Ldef3}
\end{align}
\end{small}%
Eq~\ref{eq:Ldef1} means that there are $c$ perturbed indices sampled in $\outcome$.
$\diffu$ (and $\diffv$) in Eq~\ref{eq:Ldef3} counts how many features the sampled and the clean data (the perturbed data) differ on.
The number of possible subspaces $\subspace_{c,t}$, which are disjoint by definition, is $O(k^2d)$ because $0\le c \le k$ and $|t| \le (k+1)d$.

% \aws{ex can be removed} 
% \begin{example}
% \label{exp: partition}
% Consider the dataset and the distribution $\mu$ in \Cref{exp: distribution} and suppose that the attacker perturbs one image in the training set by flipping one feature. 
% There are four outcomes of selection, which example to select and whether to flip the only feature in the selected example. 
% One possible outcome, denoted as $\outcome_1$, is that we select a clean example ($c=0$), and the only feature in this example is not flipped~($\diffu = \diffv = 0$). 
% Similarly, $\outcome_2$ can be a clean example ($c=0$) with the feature flipped~($\diffu = \diffv = 1$). 
% We have $\cleandistmass{\outcome_1} = \poisondistmass{\outcome_1} = \frac{1}{2} \times \symbolremain = 0.4$ and $\cleandistmass{\outcome_2} = \poisondistmass{\outcome_2} = \frac{1}{2} \times (1-\symbolremain) = 0.1$. 
% So we group these two outcomes in $\subspace_{0,0}$ in the definition above because $\eta(\outcome_1)=\eta(\outcome_2)=1$ (\Cref{exp: merge} shows a similar case).
% The probabilities of other subspaces can be found in \Cref{exp: lemma}, namely, $\subspace_1 = \subspace_{1,1}$ and $\subspace_3 = \subspace_{1,-1}$.
% \end{example}

% We then compute the likelihood of $\outcome \sim \selectflip(\poisoned{D}, \poisoned{\bfxtest})$ being in the non-empty subspace $\subspace(c,u,v)$.
% \begin{align}
%     &\underset{\outcome\sim \selectflip(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left(\outcome \in \subspace(c, u, v)\right) = |\subspace(c, u, v)| \frac{1}{n^k}b^ua^{(k+1)d-u}, \label{eq:prd''}
% \end{align}
% \begin{align}
%     &\underset{\outcome\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left(\outcome \in \subspace(c, u, v)\right) \nonumber\\
%     =& \sum_{\outcome \in L(c,u,v)} \underset{\outcome\sim \mu(\poisoned{D}, \poisoned{\bfxtest})}{\PP}\left(\outcome = \outcome\right)\nonumber \\
%     =& |\subspace(c, u, v)| \frac{1}{n^k}b^ua^{(k+1)d-u}, \label{eq:prd''}
% \end{align}
% where $|\subspace(c, u, v)|$ is the size of subspace $\subspace(c, u, v)$.
% Similarly, we have
% \begin{align}
%     \underset{\outcome \sim \selectflip(D,\bfxtest)}{\PP}\left(\outcome \in \subspace(c, u, v)\right) =|\subspace(c, u, v)|\frac{1}{n^k}b^va^{(k+1)d-v} \label{eq:prd'}
% \end{align}

% \aws{can we give b and a more descriptive names -- also b is a function of a. So maybe use the same symbol.} \yh{made some changes so that they only appear in this theorem.}
The next theorems show how to compute the likelihood ratio of $\subspace_{c,t}$ and $\cleandistmass{\subspace_{c, t}}$.

\begin{theorem}[Compute $\eta_{c, t}$]
\label{thm:selectflip_main1}
% The likelihood ratio $\eta_{c, t}$ of a non-empty subspace $\subspace_{c,t}$ is
$\eta_{c,t} = \cleandistmass{\subspace_{c, t}}/ \poisondistmass{\subspace_{c, t}}  = (\symbolflip / \symbolremain)^{t}$, 
where $\symbolflip$ and $\symbolremain$ are parameters controlling the noise level in \technique's smoothing distribution $\mu$. 
\end{theorem}

\begin{theorem}[Compute $\cleandistmass{\subspace_{c, t}}$]
\label{thm:selectflip_main2}
\begin{align*}
   \cleandistmass{\subspace_{c, t}} = \underset{\outcome \sim \cleandist}{\PP}(\outcome \text{ satisfies Eq~\ref{eq:Ldef1}}) \underset{\outcome \sim \cleandist}{\PP}(\outcome \text{ satisfies Eq~\ref{eq:Ldef3}} \mid \outcome \text{ satisfies Eq~\ref{eq:Ldef1}}),
\end{align*}
where $\PP_{\outcome \sim \cleandist}(\outcome \text{ satisfies Eq~\ref{eq:Ldef1}}) = \mathrm{Binom}(c;k,\frac{\poisonins}{n})$ is the PMF of the binomial distribution and 
\begin{small}
\begin{align}
    T(c,t) \triangleq \underset{\outcome \sim \cleandist}{\PP}(\outcome \text{ satisfies Eq~\ref{eq:Ldef3}} \mid \outcome \text{ satisfies Eq~\ref{eq:Ldef1}}) = \sum_{\substack{0 \le \diffu_i, \diffv_i \le d, \forall i\in[0,d] \\ \diffu_0-\diffv_0 + \ldots + \diffu_c-\diffv_c = t}} \prod_{i=0}^c L(\diffu_i,\diffv_i;\poisonfeat, d)\symbolflip^{\diffu_i}\symbolremain^{d-\diffu_i},\label{eq:prd'}
\end{align}
\end{small}%
where $L(\diffu,\diffv;\poisonfeat, d)$ is the same quantity defined in \citet{tightflipbound}.
\end{theorem}

% \aws{This remark is interesting because we don't know what D,x is. We should mention this idea early} \yh{We can actually compute the following quantity as in the above theorem as well because we have already made the assumption of D and x.}

\begin{remark}
We can compute $\poisondistmass{\subspace_{c, t}}$ as $\eta_{c,t}\cleandistmass{\subspace_{c, t}}$ by the definition of $\eta_{c,t}$.
\end{remark}

% \aws{what is T(..); first time it shows up}. \yh{It is actually hide in the previous theorem... but I need to define $T(c,t)$ anyway before or here.}
\textbf{Efficient algorithm to compute Eq~\ref{eq:prd'}.}
The following algorithm computes $T(c,t)$ efficiently in time~$O(d^3 + k^2d^2)$: 1) Computing $L(u, v;\poisonfeat, d)$ takes $O(d^3)$ (see \Cref{sec: proofs} for details). 2) Computing $T(0,t)$ by the definition in Eq~\ref{eq:prd'} takes $O(kd^2)$. 3) Computing $T(c,t)$ for $c\ge 1$ by the following equation takes $O(k^2d^2)$.
\begin{small}
    \begin{align}
        T(c, t) = \sum_{t_1=\max(-d, t-cd)}^{\min(d, t+cd)} T(c-1,t - t_1)T(0,t_1) \label{eq:efficient_tct}
    \end{align}
\end{small}%

\begin{theorem}[Correctness of the Algorithm]
\label{thm:selectflip_tct}
$T(c,t)$ in Eq~\ref{eq:efficient_tct} is the same as the one in Eq~\ref{eq:prd'}.
\end{theorem}





% \paragraph{Extending to perturbation functions $\featfliplabelflip$ and $\labelflip$}
The above computation still applies to perturbation function $\featfliplabelflip$ and $\labelflip$. 
Intuitively, flipping the label can be seen as flipping another dimension in the input features (Details in \Cref{sec: other_perturbs}). 


\textbf{Practical perspective.} For each test input $\bfxtest$, we need to estimate $\firstp$ for the smoothed algorithm $\salg$ given the benign dataset $D$.
We use Monte Carlo sampling to compute $\firstp$ by the Clopper-Pearson interval.
We also reuse the trained algorithms for each test input in the test set by using \textit{Bonferroni correction}.
We memoize the certified radius by enumerating all possible $\firstp$ beforehand so that checking Eq~\ref{eq:certgoal1} can be done in constant time in an online scenario (details in \Cref{sec: appendix_practical}).
We cannot use floating point numbers because some intermediate values are too small to store in the floating point number format. 
Instead, we use rational numbers which represent the nominator and denominator in large numbers.


==> BagFlip_ A Certified Defense against Data Poisoning/tables/approaches.tex <==
\begin{table}[t]
    \centering
    \caption{This paper compared to other approaches. RAB~\cite{RAB} can handle perturbation $\featflip^*$ that perturbs the input within a $l_2$-norm ball of radius $\poisonfeat$.}
    % \setlength{\tabcolsep}{1pt}
 \renewcommand{\arraystretch}{1}
    \begin{small}
    \begin{tabular}{llllc}
        \toprule
         Approach & Perturbation $\perturb$ & Probability measure $\mu$ & Goal\\ 
        \midrule
        \citet{bagging, framework_def} & Any & Bagging  & Trigger-less \\
        % DPA~\cite{partitioning} & Any & N/A & Deterministic & \xmark  \\
        \citet{labelflip} & $\labelflip$ & Noise  & Trigger-less  \\
        RAB~\cite{RAB} & $\featflip^*$ & Noise  & Trigger-less, Backdoor  \\
        \citet{featureflip} & $\featfliplabelflip, \featflip, \labelflip$ & Noise  & Trigger-less, Backdoor  \\
        \emph{This paper} & $\featfliplabelflip, \featflip, \labelflip$ & Bagging+Noise & Trigger-less, Backdoor \\
        \bottomrule
    \end{tabular}
    \end{small}
    \vspace{-1em}
    \label{tab:approaches}
\end{table}


==> BagFlip_ A Certified Defense against Data Poisoning/tables/backdoor_res.tex <==
\centering
\caption{Compared to FeatFlip on $\featfliplabelflipone$ and RAB $\featflipone$ with normal accuracy~(Acc.) and certified accuracy at different poisoning amount $\assumeradii$~(CF@$\assumeradii$).
% We show the best configuration of \technique and RAB (see full results in \Cref{sec: appendix_res}).
}
\setlength{\tabcolsep}{3pt}
\begin{small}
\begin{tabular}{llllll}
\toprule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize MNIST-17}} && Acc. & CF@0 & CF@0.5 & CF@1.0         \\
\cmidrule{3-6}
 &
 FeatFlip  & 98 & 36 & 0 & 0 \\
 & \technique-0.95 & 97 & \textbf{81} & \textbf{60} & 0 \\
 & \technique-0.9 & 97 & 72 & 46 & \textbf{4}\\
\midrule
 \multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize MNIST-01}} && Acc. & CF@0 & CF@1.5 & CF@3.0         \\
 \cmidrule{3-6}
%  & RAB-0.5 & 99.5 & 0 & 0 & 0\\
 & RAB & 100.0 & 74.4 & 0 & 0\\
& \technique-0.8 & 99.6 & \textbf{98.4} & \textbf{96.5} & 84.6 \\
& \technique-0.7 & 99.5 & 98.0 & 95.8 & \textbf{91.9}\\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize CIFAR10-02}}  && Acc. & CF@0 & CF@0.1 & CF@0.2         \\
\cmidrule{3-6}
 & RAB & 73.3 & 0 & 0 & 0\\
%  & RAB-2 & 65.6 & 0 & 0 & 0\\
& \technique-0.8 & 73.1 & 16.8 & 11.0 & 6.8 \\
& \technique-0.7 & 71.7 & \textbf{41.0} & \textbf{34.6} & \textbf{29.2} \\
\bottomrule
\end{tabular}
\end{small}


% \technique-0.95 (\technique-0.9) achieves 97.5\%~(97.2\%) normal accuracy and 86.5\%~(71.6\%) certified evasion accuracy against $\featfliplabelflipone$ on MNIST-17, respectively, while FeatFlip achieves 98\% normal accuracy and 82\% certified evasion accuracy~($\assumeradii=0$).
% The certified accuracy of \technique-0.95 (\technique-0.9) retains 78.7\%~(54.1\%) at $\assumeradii=50$, respectively.
% FeatFlip achieves 36\% certified accuracy at $\assumeradii=1$ and its certified accuracy drops to zero after $\assumeradii=3$.

% On MNIST-01, \technique-0.8~(\technique-0.7) achieves 99.6\%~(99.5\%, respectively) normal accuracy, which is similar compared to RAB-1's 100\% and RAB-2's 99.5\%.
% \technique-0.8~(\technique-0.7) achieves 98.4\%~(98.0\%, respectively) certified evasion accuracy, which is much higher than RAB-0.5's 0\% and RAB-1's 74.4\%.
% \technique-0.8~(\technique-0.7) retains 83.7\%~(91.5\%, respectively) certified accuracy at $\assumeradii=400$, while the both configurations of RAB's certified accuracy drops to zero after $\assumeradii=1$.
% We observe similar results on CIFAR10-02 and present the details in supplementary materials.
% We observe similar results on CIFAR10-02.
% \technique-0.8~(\technique-0.7) achieves 74.3\%~(73.3\%, respectively) normal accuracy, which is similar compared to RAB-1's 73.3\% and much higher than RAB-2's 65.6\%.
% \technique-0.8~(\technique-0.7) achieves 16.8\%~(41.0\%, respectively) certified evasion accuracy, while the both configurations of RAB's certified accuracy drops to zero after $\assumeradii=0$.
% \technique-0.7 still retains 23.8\% certified accuracy at $\assumeradii=30$.

==> BagFlip_ A Certified Defense against Data Poisoning/tables/backdoor_res_full.tex <==
\centering
\caption{Compared to FeatFlip on $\featfliplabelflipone$ and RAB $\featflipone$ with normal accuracy~(Acc.) and certified accuracy at different poisoning amount $\assumeradii$~(CF@$\assumeradii$).
% We show the best configuration of \technique and RAB (see full results in \Cref{sec: appendix_res}).
}
\setlength{\tabcolsep}{3pt}
\begin{small}
\begin{tabular}{llllll}
\toprule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize MNIST-17}} && Acc. & CF@0 & CF@0.5 & CF@1.0         \\
\cmidrule{3-6}
 &
 FeatFlip  & 98 & 36 & 0 & 0 \\
 & \technique-0.95 & 97 & \textbf{87} & \textbf{75.3} & \textbf{26.3} \\
 & \technique-0.9 & 97 & 72 & 45.9 & 3.6\\
\midrule
 \multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize MNIST-01}} && Acc. & CF@0 & CF@1.5 & CF@3.0         \\
 \cmidrule{3-6}
 & RAB-0.5 & 99.5 & 0 & 0 & 0\\
 & RAB & 100.0 & 74.4 & 0 & 0\\
& \technique-0.8 & 99.6 & \textbf{98.4} & \textbf{96.5} & 84.6 \\
& \technique-0.7 & 99.5 & 98.0 & 95.8 & \textbf{91.9}\\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize CIFAR10-02}}  && Acc. & CF@0 & CF@0.1 & CF@0.2         \\
\cmidrule{3-6}
 & RAB & 73.3 & 0 & 0 & 0\\
 & RAB-2 & 65.6 & 0 & 0 & 0\\
& \technique-0.8 & 73.1 & 16.8 & 11.0 & 6.8 \\
& \technique-0.7 & 71.7 & \textbf{41.0} & \textbf{34.6} & \textbf{29.2} \\
\bottomrule
\end{tabular}
\end{small}


% \technique-0.95 (\technique-0.9) achieves 97.5\%~(97.2\%) normal accuracy and 86.5\%~(71.6\%) certified evasion accuracy against $\featfliplabelflipone$ on MNIST-17, respectively, while FeatFlip achieves 98\% normal accuracy and 82\% certified evasion accuracy~($\assumeradii=0$).
% The certified accuracy of \technique-0.95 (\technique-0.9) retains 78.7\%~(54.1\%) at $\assumeradii=50$, respectively.
% FeatFlip achieves 36\% certified accuracy at $\assumeradii=1$ and its certified accuracy drops to zero after $\assumeradii=3$.

% On MNIST-01, \technique-0.8~(\technique-0.7) achieves 99.6\%~(99.5\%, respectively) normal accuracy, which is similar compared to RAB-1's 100\% and RAB-2's 99.5\%.
% \technique-0.8~(\technique-0.7) achieves 98.4\%~(98.0\%, respectively) certified evasion accuracy, which is much higher than RAB-0.5's 0\% and RAB-1's 74.4\%.
% \technique-0.8~(\technique-0.7) retains 83.7\%~(91.5\%, respectively) certified accuracy at $\assumeradii=400$, while the both configurations of RAB's certified accuracy drops to zero after $\assumeradii=1$.
% We observe similar results on CIFAR10-02 and present the details in supplementary materials.
% We observe similar results on CIFAR10-02.
% \technique-0.8~(\technique-0.7) achieves 74.3\%~(73.3\%, respectively) normal accuracy, which is similar compared to RAB-1's 73.3\% and much higher than RAB-2's 65.6\%.
% \technique-0.8~(\technique-0.7) achieves 16.8\%~(41.0\%, respectively) certified evasion accuracy, while the both configurations of RAB's certified accuracy drops to zero after $\assumeradii=0$.
% \technique-0.7 still retains 23.8\% certified accuracy at $\assumeradii=30$.

==> BagFlip_ A Certified Defense against Data Poisoning/tables/symbols.tex <==
\begin{table}[t]
    \centering
    \caption{Symbols in Section~\ref{sec: featflip}.}
    % \setlength{\tabcolsep}{1pt}
 \renewcommand{\arraystretch}{1}
    \begin{small}
    \begin{tabular}{cl}
        \toprule
         Symbol & Explanation\\ 
        \midrule
        % $\poisonins$ & The number of poisoned examples in training set.  \\
        % $\poisonfeat$ & The number of poisoned features per example.  \\
        $k$ & The number of the examples selected for training each classifier.\\
        $d$ & The number of features. \\
        $n$ & The size of the training set.\\
        % $\outcome$ & A concrete sample containing the smoothed dataset and test example from $\selectflip$. \\
        $c$ & The number of poisoned indices in the smoothed dataset. \\ 
        \multirow{2}{*}{$t$} & $t=\diffu-\diffv$, where $\diffu$ (and $\diffv$, respectively) counts the number of different features between the\\
        & smoothed data and the clean data (the poisoned data, respectively).\\
        % $F$ & PMF of binomial distribution.\\
        $\symbolremain$ & A parameter controlling the probability of a feature remaining the same. \\
        % $K$ & The number of categories in each feature. \\
        \multirow{2}{*}{$\symbolflip$} & A parameter controlling the probability of a feature flipping to a different feature. $\symbolflip = \frac{1-\symbolremain}{K}$, \\ 
        & where $K$ is the number of other categories in each feature.\\
        \bottomrule
    \end{tabular}
    \end{small}

    \label{tab:symbols}
\end{table}


==> BagFlip_ A Certified Defense against Data Poisoning/tables/trigger_less_res.tex <==
\begin{table}
\centering
\caption{Certified accuracy on MNIST and EMBER with perturbations $\featflipone$ and $\featflipinf$. Note that the certified accuracies are the same poisoning amount $R=0$  because we reuse the trained models. }
\setlength{\tabcolsep}{3pt}
\begin{small}
\begin{tabular}{llllllllllllll}
\toprule
            && \multicolumn{6}{c}{$\featflipone$}                 & \multicolumn{6}{c}{$\featflipinf$}        \\ 
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
\multirow{4}{*}{\rotatebox[origin=c]{90}{MNIST}} &$\assumeradii$   & $0$ & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $0$ & $0.13$ & $0.27$ & $0.40$ & $0.53$ & $0.83$  \\
\cmidrule{2-14}
 & Bagging     & \textbf{94.54}           & 66.84& 0    & 0    & 0     & 0     & \textbf{94.54} & \textbf{90.83} &	\textbf{85.45} &	77.61 &	61.46 & 0     \\
 & Bagging-0.9     & 93.58     & 71.11     & 0         & 0        & 0   & 0    & 93.58     & 89.80 & 84.92 & \textbf{78.60} & \textbf{68.11} & 0 \\
% Bagging     & 94.83           & 68.69& 0    & 0    & 0     & 0     & 94.83 & 91.22            & 86.50& 78.82& 63.34& 0     \\
& \technique-0.9 & 93.62           & \textbf{75.95} & 27.73& 4.02 & 0     & 0     & 93.62 & 89.45            & 83.62& 74.19& 56.65& 0     \\
& \technique-0.8 & 90.72           & 73.94& \textbf{46.20} & \textbf{33.39} & \textbf{24.23} & \textbf{5.07}  & 90.72 & 84.11            & 74.50& 60.56& 39.21& 0    \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{EMBER}} &$\assumeradii$   & $0$ & $0.07$ & $0.13$ & $0.20$ & $0.27$ & $0.33$ & $0$ & $0.05$ & $0.10$ & $0.15$ & $0.20$ & $0.25$  \\
\cmidrule{2-14}
 & Bagging & \textbf{82.65} & 75.11 & 66.01 & 0 & 0 & 0
& \textbf{82.65} & 76.30 & 72.94 & 61.78 & 0 & 0\\
& Bagging-0.95      & 79.06     & 75.32     & \textbf{70.19} & 14.74     & 0    & 0    & 79.06     & 76.23     &  \textbf{73.50} & \textbf{68.45} & 14.74     & 0     \\
& \technique-0.95 & 79.17 & \textbf{75.93} & 69.30 & \textbf{57.36} & 0 & 0
& 79.17 & \textbf{76.83} & 72.41 & 62.04 & \textbf{30.36} & 0\\
& \technique-0.9 & 78.18 & 69.40 & 62.11 & 41.21 & \textbf{13.89} & \textbf{1.70} 
& 78.18 & 70.79 & 63.16 & 41.24 & 11.64 & 0\\
\bottomrule
\end{tabular}
\end{small}
\label{tab:trigger_less_res}
\vspace{-1em}
\end{table}

==> sections/legacy.tex <==
\subsubsection{Bound by the KL divergence}
\begin{theorem}
\label{thm:KL_bound}
Consider the binary classification case where $|\mathcal{C}|=2$,
Denote $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'', x)=y^*)$ as $p$, Eq~\ref{eq:certgoal1} holds if 
\begin{align}
    \poisonfeat \poisonins < \dfrac{|D|\log(4p(1-p))}{2k\log(\frac{b}{a})(a-b)},
\end{align}
where $\poisonins$ is the number of the poisoned instances, $\poisonfeat$ is the number of the poisoned features, $k$ is the size of each bag, and $a, b$ are the probability of a featuring remaining the same and being flipped. 
\end{theorem}
% \todo{It seems $T=(a-b)\poisonfeat$, prove that.}

\begin{lemma}
\label{lemma:T}
Define $T$ as
\begin{align}
    T = \sum_{u=0}^d \sum_{v=0}^d |L(u,v;\poisonfeat)| b^u a^{d-u} (v-u)\label{eq:defofT}
\end{align}
and similarly in the Lemma 5 of \citet{tightflipbound}, $|L(u,v;\poisonfeat)|$ is defined as,
\[\sum_{i=\max(0,v-\poisonfeat)}^{\min(u, d-\poisonfeat, \lfloor \frac{u+v-\poisonfeat}{2} \rfloor)} (K-1)^j \binom{\poisonfeat}{j} \binom{\poisonfeat-j}{u-i-j} K^i \binom{d-\poisonfeat}{i},\]
where $j=u+v-2i-\poisonfeat$.
Then 
\[T = (a-b)s\]
\end{lemma}



\textbf{Proof of the Theorem~\ref{thm:KL_bound}.}
\begin{proof}
Denote $D'\sim \mu(D)$ and $D''\sim \mu(\poisoned{D})$, from the theorem in Example 5 of \cite{labelflip}, Eq~\ref{eq:certgoal1} holds if 
\begin{align}
    \KL(D''\|D') < -\frac{1}{2}\log(4p(1-p)) \label{eq:KLproof0}
\end{align}
We now calculate the KL divergence between the distribution generated from the poisoned dataset $\poisoned{D}$ and the distribution generated from the original dataset $D$.
\begin{align}
    &\KL(D''\|D') \nonumber\\
    = &k \KL(D''_1\|D'_1)\label{eq:KLproof1}\\
    = &k \sum_{w=1}^{|D|} \sum_{\bfx} p_{D_1''}(w, \bfx) \log\frac{p_{D_1''}(w, \bfx)}{p_{D_1'}(w, \bfx)}\nonumber\\
    = &k \sum_{w \in \poisoned{I}} \sum_{\bfx} p_{D_1''}(w, \bfx) \log\frac{p_{D_1''}(w, \bfx)}{p_{D_1'}(w, \bfx)}\label{eq:KLproof2}\\
    \le &k\poisonins \sum_{\bfx} \frac{a^d}{|D|}  \left(\frac{b}{a}\right)^{g(\bfx, \poisoned{D}_w)} \log\frac{b}{a} (g(\bfx, \poisoned{D}_w) - g(\bfx, D_w))\nonumber\\
    = & kp_\poisonins a^d \log(\frac{b}{a}) \sum_{\bfx}  \left(\frac{a}{b}\right)^{g(\bfx, \poisoned{D}_w)} (g(\bfx, D_w) - g(\bfx, \poisoned{D}_w))\label{eq:KLproof3}
\end{align}
where $\poisoned{I}$ are the set of poisoned indices, $\KL(D_1'' \| D_1')$ is the KL divergence of the first selected instance.
We have Eq~\ref{eq:KLproof1} because each selected instance is independent. 
We have Eq~\ref{eq:KLproof2} because the $p_{D''_1}(w, \bfx)$ and $p_{D'_1}(w, \bfx)$ only differs when the $w$th instance is poisoned.

The attacker can modify $\poisoned{D}_w$ to maximize Eq~\ref{eq:KLproof3}. And the Lemma 4 in \citet{tightflipbound} states that the maximal value is achieved when $\poisoned{D}_w$ has exact $\poisonfeat$ features flipped to another value. Because the independence of the features, it does not matter which of them are flipped.

Now suppose the first $\poisonfeat$ features are flipped in $\poisoned{D}_w$, we then need to compute Eq~\ref{eq:KLproof3}. 
If we denote $g(\bfx, \poisoned{D}_w)$ as $u$ and $g(\bfx, D_w)$ as $v$, and we count the size of the set $L(u,v;\poisonfeat)=\{\bfx \mid g(\bfx, \poisoned{D}_w) = u, g(\bfx, D_w) = v\}$, then we can compute Eq~\ref{eq:KLproof3} as
\begin{align*}
   kp_\poisonins a^d \log(\frac{a}{b}) \sum_{u=0}^d \sum_{v=0}^d |L(u,v;\poisonfeat)| \left(\frac{b}{a}\right)^{u}(v-u) 
\end{align*}
Let $T$ be defined as in Eq~\ref{eq:defofT}, we then have
\begin{align}
    \KL(D'' \| D') = kp_\poisonins \log(\frac{a}{b})T \label{eq:KLproof4}
\end{align}
Combine Eq~\ref{eq:KLproof0}, Eq~\ref{eq:KLproof4}, and Lemma~\ref{lemma:T}, we have 
\begin{align*}
    kp_\poisonins \log(\frac{a}{b})(a-b)\poisonfeat <& -\frac{1}{2}\log(4p(1-p))\\
    \poisonins \poisonfeat <& \dfrac{|D|\log(4p(1-p))}{2k\log(\frac{b}{a})(a-b)}
\end{align*}
\end{proof}

\textbf{Proof of the Lemma~\ref{lemma:T}.}
\begin{proof}
Notice that the value of $T$ does not defend on the feature dimension $d$. 
Thus, we prove the lemma by induction on $d$.
We further denote the value of $T$ under the feature dimension $d$ as $T_d$.

\textbf{Base case.} Because $0 \le s \le d$, when $d = 0$, it is easy to see $T_0 = s(a-b) = 0$.

\textbf{Induction case.} 
We first prove $T_{d+1}=s(a-b)$ under a special case, where $s = d+1$, given the inductive hypothesis $T_d = s(a-b)$ for all $s = d$. 

By definition
\begin{align}
    T_{d+1} = \sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u,v;\poisonfeat;d+1)| b^u a^{d+1-u} (v-u),\label{eq:lemmaT0}
\end{align}
where we denote $L(u,v;\poisonfeat)$ as $L(u,v;\poisonfeat;d+1)$ when feature dimension is $d+1$.

By the definition of $L(u,v;\poisonfeat)$, we have the following equation when $0 \le s \le d$
\begin{align}
    |L(u,v;d+1;d+1)| = (K-1)|L(u-1,v-1;d;d)| +\nonumber\\ |L(u-1,v;d;d)| + |L(u,v-1;d;d)|\label{eq:lemmaT4}
\end{align}
and 
\begin{align}
    \sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^u a^{d-u} = 1\label{eq:lemmaT8}
\end{align}
Plug Eq~\ref{eq:lemmaT4} into Eq~\ref{eq:lemmaT0}, we have the following equations when $s = d+1$,
\begin{align}
    T_{d+1} = &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} (K-1)|L(u-1,v-1;d;d)|b^u a^{d+1-u} (v-u) + \nonumber\\
    &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u-1,v;d;d)| b^u a^{d+1-u}  (v-u)+\nonumber\\
    &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u,v-1;d;d)| b^u a^{d+1-u} (v-u)\nonumber\\
    = &b(K-1)\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)|b^u a^{d-u} (v-u) + \label{eq:lemmaT5}\\
    &b\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^{u} a^{d-u} (v-u-1)+\label{eq:lemmaT6}\\
    &a\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^{u} a^{d-u} (v-u+1)\label{eq:lemmaT7}\\
    = & \sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;d;d)| b^{u} a^{d-u} [(v-u) + (a-b)] \nonumber\\
    = &d(a-b) + (a-b)\label{eq:lemmaT9}\\
    = &\poisonfeat(a-b)\nonumber
\end{align}
We have Eq~\ref{eq:lemmaT4}, Eq~\ref{eq:lemmaT5} and Eq~\ref{eq:lemmaT6} because $L(u,v;\poisonfeat,d)=0$ when $u>d$, $v>d$, $u<0$ , or $v<0$.
We have Eq~\ref{eq:lemmaT9} by plugging in Eq~\ref{eq:lemmaT8}.

Next, we are going to show that $T_{d+1} = s(a-b)$ for all $0 \le s \le d$, given the inductive hypothesis $T_d = s(a-b)$ for all $0 \le s \le d$. 

By the definition of $L(u,v;\poisonfeat)$, we have the following equations when $0 \le s \le d$
\begin{align}
    |L(u,v;\poisonfeat;d+1)| = |L(u,v;\poisonfeat;d)| + K|L(u-1,v-1;\poisonfeat;d)|\label{eq:lemmaT1}
\end{align}
Plug Eq~\ref{eq:lemmaT1} into Eq~\ref{eq:lemmaT0}, for all $0 \le s \le d$, we have
\begin{align}
    T_{d+1} = &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} |L(u,v;\poisonfeat;d)|b^u a^{d+1-u} (v-u) + \nonumber\\
    &\sum_{u=0}^{d+1} \sum_{v=0}^{d+1} K|L(u-1,v-1;\poisonfeat;d)| b^u a^{d+1-u} (v-u)\nonumber\\
    = &a\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;\poisonfeat;d)|b^u a^{d-u} (v-u) + \label{eq:lemmaT2}\\
    &bK\sum_{u=0}^{d} \sum_{v=0}^{d} |L(u,v;\poisonfeat;d)| b^{u} a^{d-u} (v-u)\label{eq:lemmaT3}\\
    = & as(a-b) + bKs(a-b) \nonumber\\
    = &s(a-b)\nonumber
\end{align}
We have Eq~\ref{eq:lemmaT2} and Eq~\ref{eq:lemmaT3} because $L(u,v;\poisonfeat,d)=0$ when $u>d$, $v>d$, $u<0$ , or $v<0$.


\end{proof}

% The following bound is quite loose, but it makes easier to understand the relation between parameters. 
% \begin{corollary}
% \label{coro:KL}
% Eq~\ref{eq:certgoal1} holds if 
% \begin{align}
%     \poisonfeat < \dfrac{\log(4p(1-p))}{2k\log(\frac{b}{a})p_\poisonins}
% \end{align}
% \end{corollary}
% We get the above corollary because we can derive an upper bound of $T$ as $\poisonfeat$.


% \begin{proof}
% Notice that an upper bound of Eq~\ref{eq:KLproof3} is 
% \begin{align}
%     &kp_\poisonins a^d \log(\frac{b}{a}) \sum_{\bfx} \left(\frac{b}{a}\right)^{g(\bfx, \poisoned{D}_w)}(-\poisonfeat) \nonumber\\
%     =& kp_\poisonins a^d \log(\frac{a}{b})\poisonfeat \sum_{\bfx}  \left(\frac{b}{a}\right)^{g(\bfx, \poisoned{D}_w)}\nonumber\\
%     =& kp_\poisonins a^d \log(\frac{a}{b})\poisonfeat \sum_{i=0}^d \binom{d}{i} K^i \left(\frac{b}{a}\right)^i \nonumber \\
%     =& kp_\poisonins a^d \log(\frac{a}{b})\poisonfeat (1 + \frac{Kb}{a})^d \nonumber\\
%     =& kp_\poisonins \log(\frac{a}{b})\poisonfeat, \label{eq:coro1proof0}
% \end{align}
% because the attacker can flip at most $\poisonfeat$ features, then $g(\bfx, \poisoned{D}_w)-g(\bfx, D_w)$ is lower bounded by $-\poisonfeat$ (notice that $\log(\frac{b}{a})$ is negative).
% Combine Eq~\ref{eq:KLproof0} and Eq~\ref{eq:coro1proof0}, we have 
% \begin{align*}
%     kp_\poisonins\log(\frac{a}{b})\poisonfeat <& -\frac{1}{2}\log(4p(1-p))\\
%     \poisonfeat <& \dfrac{\log(4p(1-p))}{2k\log(\frac{b}{a})p_r}
% \end{align*}
% \end{proof}

\begin{corollary}
\label{coro:KL_cert}
From Theorem~\ref{thm:KL_bound}, we can compute the certified radius $R_{cert}(\poisonins)$ as
\begin{align}
    R_{cert}(\poisonins) = \min(d, \lceil \dfrac{|D|\log(4p(1-p))}{2k\log(\frac{1-a}{aK})\frac{a(K+1)-1}{K}\poisonins} \rceil - 1) \label{eq:cert_radius}
\end{align}
\end{corollary}

\begin{remark}
From Eq~\ref{eq:cert_radius}, we know that the certified radius becomes larger when the classifiers accuracy $p$ is larger, the number of instances in the bag $k$ is smaller, the probability of remaining the same $a$ is smaller, the number of categories of each feature $K$ is smaller, or the number of poisoned instances $\poisonins$ is smaller.

However, there is a trade-off between $p$ and $a$ because the more noise is added to the training set, the lower the performance of each classifier gets. 
There is also a trade-off between $p$ and $k$ because the less instances is in the bag, the lower the performance of each classifier gets.
\end{remark}

% \begin{remark}
% Note that, if the features are not categorized, the category number $K$ can still be upper bounded by $|D|$ because each feature has at most $|D|$ different values in the training set, as we can randomly flip each feature to an existing features in the bag. Then the certified radius $R_{cert}(\poisonins)$ can be computed as
% \begin{align*}
%     R_{cert}(\poisonins) = \max(d, \lceil \dfrac{\log(4p(1-p))|D|^2}{2k\log(\frac{1-a}{a|D|})\poisonins} \rceil - 1) 
% \end{align*}
% \end{remark}

\subsubsection{Combine the Neyman-Pearson Lemma and the KL divergence}
As in the previous sections, we show an efficient relaxation of the bound computed by the Neyman-Pearson Lemma. 
The relaxation simply ignores all subspaces $\mathcal{L}^{l+1}(\bfc, \bfu, \bfv),\mathcal{L}^{l+2}(\bfc, \bfu, \bfv),\ldots, \mathcal{L}^k(\bfc, \bfu, \bfv)$.
However, we can get a tighter bound by applying the KL divergence bound to the ignored subspaces. 
\begin{lemma}
The KL divergence between $\mu(\poisoned{D})$ and $\mu(D)$ on the subspace $\bigcup_{i=l+1}^k \mathcal{L}^i(\bfc, \bfu, \bfv)$ is 
\[(kp_\poisonins - lp_\poisonins + l)\log(\frac{a}{b})T\]
\end{lemma}

\begin{lemma}
\label{lemma:extendedKL}
Consider the binary classification case, denoting $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'', x)=y^*)$ as $p$, 
\begin{align*}
    (1-\lambda)\underset{D'\sim \mu(D)}{\PP}(f(D', x)=y^*) > \lambda\underset{D'\sim \mu(D)}{\PP}(f(D', x)=y)
\end{align*}
holds for all $y \neq y^*$ if 
\begin{align*}
    \mathrm{KL}(D''\| D') < \log(\frac{(1-\lambda)p}{\lambda(1-p)})(1-\lambda) - \log(\frac{p}{\lambda})
\end{align*}
Specifically, if we consider the subspace $\bigcup_{i=l+1}^k \mathcal{L}^i(\bfc, \bfu, \bfv)$, then
\begin{align}
    (kp_\poisonins - lp_\poisonins + l)\log(\frac{a}{b})T < \log(\frac{(1-\lambda)p}{\lambda(1-p)})(1-\lambda) - \log(\frac{p}{\lambda})\label{eq:generalKL}
\end{align}
\end{lemma}

\begin{remark}
Lemma~\ref{lemma:extendedKL} is a more general KL divergence bound and \citet{divergences} provided a special case when $\lambda=\frac{1}{2}$, which is used in Theorem~\ref{thm:KL_bound}. 
We need the general version for the following theorem.
\end{remark}

\begin{theorem}
Consider the binary classification case, denoting $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'', x)=y^*)$ as $p$ and choosing $l$ for computing the feasible Neyman-Pearson bound, Eq~\ref{eq:certgoal1} holds if for all $\gamma \in [0, 1 - F(l;k,p_\poisonins)]$,
\begin{align}
    \mathrm{NP_{bound}}(\frac{p-\gamma}{F(l;k,p_\poisonins)})F(l;k,p_\poisonins) +\nonumber\\ \mathrm{KL_{bound}}(\frac{\gamma}{1 - F(l;k,p_\poisonins)})(1-F(l;k,p_\poisonins)) \ge \frac{1}{2},
\end{align}
where $\mathrm{NP_{bound}}(z)$ computes the lower bound $lb_l$ when $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'',x)=y^*)$ is set to $z$ and $\mathrm{KL_{bound}}(z)$ computes the largest $\lambda$ satisfying Eq~\ref{eq:generalKL} when $\underset{D''\sim \mu(\poisoned{D})}{\PP}(f(D'',x)=y^*)$ is set to $z$.
\end{theorem}

\subsection{Compare to the bagging and the feature-flipping approach}
We compare the certified radius computed from Corollary~\ref{coro:KL_cert} to the certified radius computed from the bagging approach~\cite{bagging} and the feature-flipping approach~\cite{featureflip}.

We look at a realistic dataset MNIST 1/7 dataset ($d=28*28+1=785$, i.e., we also consider label-flipping attack) that just includes digits 1 and 7. This subset includes 13,007 training examples ($|D|=13007$) and 2,163 testing examples. 
In \citet{bagging}, they choose the bagging size $k=50$ and the probability $a=0.7$. 
Also, we assume that the classifier performance $p=0.8$ because the task is relatively easy. And we will further justify this aspect in the experiment section.

From Corollary 1 in~\citet{bagging}, we can compute $R_{bag}=92$.
From the experiment section in~\citet{featureflip}, we use an upper bound of $R_{ff}=3d=2355$ for comparison.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/sim_bounds}
    \caption{$R_{cert}$ computed by three approaches.}
    \label{fig:sim_bounds}
\end{figure}

\todo{Wrong!} Figure~\ref{fig:sim_bounds} shows the results of $R_{cert}$ computed by three approaches. 
Our approach can certify up to $\poisonins=1135$ poisoned instances modified in the training set assuming the attacker can flip all features in the instance (i.e., $R_{cert}(1135)=d$). And our approach can certify up to $\poisonfeat=68$ features being flipped assuming the attacker can modify all instances in the training set (i.e., $R_{cert}(|D|)=68$).

\begin{remark}
Notice that this result is based on the assumption that we can achieve a classifier performance $p=0.8$, given $k=50$ and $a=0.7$. 
However, our approach may require larger $k$ to mitigate the effect of noise and may require larger $a$ to mitigate the insufficient bagging size. 

Also, the comparison is not fair for~\citet{bagging} because the bagging approach does not assume all features are categorized. 
\end{remark}

\subsection{Certified defense of data poisoning and evasion attack}


==> tables/backdoor_res_full.tex <==
\centering
\caption{Compared to FeatFlip on $\featfliplabelflipone$ and RAB $\featflipone$ with normal accuracy~(Acc.) and certified accuracy at different poisoning amount $\assumeradii$~(CF@$\assumeradii$).
% We show the best configuration of \technique and RAB (see full results in \Cref{sec: appendix_res}).
}
\setlength{\tabcolsep}{3pt}
\begin{small}
\begin{tabular}{llllll}
\toprule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize MNIST-17}} && Acc. & CF@0 & CF@0.5 & CF@1.0         \\
\cmidrule{3-6}
 &
 FeatFlip  & 98 & 36 & 0 & 0 \\
 & \technique-0.95 & 97 & \textbf{87} & \textbf{75.3} & \textbf{26.3} \\
 & \technique-0.9 & 97 & 72 & 45.9 & 3.6\\
\midrule
 \multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize MNIST-01}} && Acc. & CF@0 & CF@1.5 & CF@3.0         \\
 \cmidrule{3-6}
 & RAB-0.5 & 99.5 & 0 & 0 & 0\\
 & RAB & 100.0 & 74.4 & 0 & 0\\
& \technique-0.8 & 99.6 & \textbf{98.4} & \textbf{96.5} & 84.6 \\
& \technique-0.7 & 99.5 & 98.0 & 95.8 & \textbf{91.9}\\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize CIFAR10-02}}  && Acc. & CF@0 & CF@0.1 & CF@0.2         \\
\cmidrule{3-6}
 & RAB & 73.3 & 0 & 0 & 0\\
 & RAB-2 & 65.6 & 0 & 0 & 0\\
& \technique-0.8 & 73.1 & 16.8 & 11.0 & 6.8 \\
& \technique-0.7 & 71.7 & \textbf{41.0} & \textbf{34.6} & \textbf{29.2} \\
\bottomrule
\end{tabular}
\end{small}


% \technique-0.95 (\technique-0.9) achieves 97.5\%~(97.2\%) normal accuracy and 86.5\%~(71.6\%) certified evasion accuracy against $\featfliplabelflipone$ on MNIST-17, respectively, while FeatFlip achieves 98\% normal accuracy and 82\% certified evasion accuracy~($\assumeradii=0$).
% The certified accuracy of \technique-0.95 (\technique-0.9) retains 78.7\%~(54.1\%) at $\assumeradii=50$, respectively.
% FeatFlip achieves 36\% certified accuracy at $\assumeradii=1$ and its certified accuracy drops to zero after $\assumeradii=3$.

% On MNIST-01, \technique-0.8~(\technique-0.7) achieves 99.6\%~(99.5\%, respectively) normal accuracy, which is similar compared to RAB-1's 100\% and RAB-2's 99.5\%.
% \technique-0.8~(\technique-0.7) achieves 98.4\%~(98.0\%, respectively) certified evasion accuracy, which is much higher than RAB-0.5's 0\% and RAB-1's 74.4\%.
% \technique-0.8~(\technique-0.7) retains 83.7\%~(91.5\%, respectively) certified accuracy at $\assumeradii=400$, while the both configurations of RAB's certified accuracy drops to zero after $\assumeradii=1$.
% We observe similar results on CIFAR10-02 and present the details in supplementary materials.
% We observe similar results on CIFAR10-02.
% \technique-0.8~(\technique-0.7) achieves 74.3\%~(73.3\%, respectively) normal accuracy, which is similar compared to RAB-1's 73.3\% and much higher than RAB-2's 65.6\%.
% \technique-0.8~(\technique-0.7) achieves 16.8\%~(41.0\%, respectively) certified evasion accuracy, while the both configurations of RAB's certified accuracy drops to zero after $\assumeradii=0$.
% \technique-0.7 still retains 23.8\% certified accuracy at $\assumeradii=30$.

==> tables/symbols.tex <==
\begin{table}[t]
    \centering
    \caption{Symbols in Section~\ref{sec: featflip}.}
    % \setlength{\tabcolsep}{1pt}
 \renewcommand{\arraystretch}{1}
    \begin{small}
    \begin{tabular}{cl}
        \toprule
         Symbol & Explanation\\ 
        \midrule
        % $\poisonins$ & The number of poisoned examples in training set.  \\
        % $\poisonfeat$ & The number of poisoned features per example.  \\
        $k$ & The number of the examples selected for training each classifier.\\
        $d$ & The number of features. \\
        $n$ & The size of the training set.\\
        % $\outcome$ & A concrete sample containing the smoothed dataset and test example from $\selectflip$. \\
        $c$ & The number of poisoned indices in the smoothed dataset. \\ 
        \multirow{2}{*}{$t$} & $t=\diffu-\diffv$, where $\diffu$ (and $\diffv$, respectively) counts the number of different features between the\\
        & smoothed data and the clean data (the poisoned data, respectively).\\
        % $F$ & PMF of binomial distribution.\\
        $\symbolremain$ & A parameter controlling the probability of a feature remaining the same. \\
        % $K$ & The number of categories in each feature. \\
        \multirow{2}{*}{$\symbolflip$} & A parameter controlling the probability of a feature flipping to a different feature. $\symbolflip = \frac{1-\symbolremain}{K}$, \\ 
        & where $K$ is the number of other categories in each feature.\\
        \bottomrule
    \end{tabular}
    \end{small}

    \label{tab:symbols}
\end{table}

